Observation of an exotic narrow doubly charmed tetraquark

Conventional hadronic matter consists of baryons and mesons made of three quarks and quark-antiquark pairs, respectively. The observation of a new type of hadronic state, a doubly charmed tetraquark containing two charm quarks, an anti-$u$ and an anti-$d$ quark, is reported using data collected by the LHCb experiment at the Large Hadron Collider. This exotic state with a mass of about 3875 MeV$/c^2$ manifests itself as a narrow peak in the mass spectrum of $D^0D^0\pi^+$ mesons just below the $D^{*+}D^0$ mass threshold. The near threshold mass together with a strikingly narrow width reveals the resonance nature of the state.

==> Authorship_LHCb-PAPER-2021-031.tex <==
% LHCb collaboration author list
% Data extracted on July 8th, 2021 at 8:38pm for paper reference LHCb-PAPER-2021-031
\centerline
{\large\bf LHCb collaboration}
\begin
{flushleft}
\small
R.~Aaij$^{32}$,
A.S.W.~Abdelmotteleb$^{56}$,
C.~Abell{\'a}n~Beteta$^{50}$,
F.J.~Abudinen~Gallego$^{56}$,
T.~Ackernley$^{60}$,
B.~Adeva$^{46}$,
M.~Adinolfi$^{54}$,
H.~Afsharnia$^{9}$,
C.~Agapopoulou$^{13}$,
C.A.~Aidala$^{87}$,
S.~Aiola$^{25}$,
Z.~Ajaltouni$^{9}$,
S.~Akar$^{65}$,
J.~Albrecht$^{15}$,
F.~Alessio$^{48}$,
M.~Alexander$^{59}$,
A.~Alfonso~Albero$^{45}$,
Z.~Aliouche$^{62}$,
G.~Alkhazov$^{38}$,
P.~Alvarez~Cartelle$^{55}$,
S.~Amato$^{2}$,
J.L.~Amey$^{54}$,
Y.~Amhis$^{11}$,
L.~An$^{48}$,
L.~Anderlini$^{22}$,
A.~Andreianov$^{38}$,
M.~Andreotti$^{21}$,
F.~Archilli$^{17}$,
A.~Artamonov$^{44}$,
M.~Artuso$^{68}$,
K.~Arzymatov$^{42}$,
E.~Aslanides$^{10}$,
M.~Atzeni$^{50}$,
B.~Audurier$^{12}$,
S.~Bachmann$^{17}$,
M.~Bachmayer$^{49}$,
J.J.~Back$^{56}$,
P.~Baladron~Rodriguez$^{46}$,
V.~Balagura$^{12}$,
W.~Baldini$^{21}$,
J.~Baptista~Leite$^{1}$,
M.~Barbetti$^{22,g}$,
R.J.~Barlow$^{62}$,
S.~Barsuk$^{11}$,
W.~Barter$^{61}$,
M.~Bartolini$^{24,h}$,
F.~Baryshnikov$^{83}$,
J.M.~Basels$^{14}$,
S.~Bashir$^{34}$,
G.~Bassi$^{29}$,
B.~Batsukh$^{68}$,
A.~Battig$^{15}$,
A.~Bay$^{49}$,
A.~Beck$^{56}$,
M.~Becker$^{15}$,
F.~Bedeschi$^{29}$,
I.~Bediaga$^{1}$,
A.~Beiter$^{68}$,
V.~Belavin$^{42}$,
S.~Belin$^{27}$,
V.~Bellee$^{50}$,
K.~Belous$^{44}$,
I.~Belov$^{40}$,
I.~Belyaev$^{41}$,
G.~Bencivenni$^{23}$,
E.~Ben-Haim$^{13}$,
A.~Berezhnoy$^{40}$,
R.~Bernet$^{50}$,
D.~Berninghoff$^{17}$,
H.C.~Bernstein$^{68}$,
C.~Bertella$^{48}$,
A.~Bertolin$^{28}$,
C.~Betancourt$^{50}$,
F.~Betti$^{48}$,
Ia.~Bezshyiko$^{50}$,
S.~Bhasin$^{54}$,
J.~Bhom$^{35}$,
L.~Bian$^{73}$,
M.S.~Bieker$^{15}$,
S.~Bifani$^{53}$,
P.~Billoir$^{13}$,
M.~Birch$^{61}$,
F.C.R.~Bishop$^{55}$,
A.~Bitadze$^{62}$,
A.~Bizzeti$^{22,k}$,
M.~Bj{\o}rn$^{63}$,
M.P.~Blago$^{48}$,
T.~Blake$^{56}$,
F.~Blanc$^{49}$,
S.~Blusk$^{68}$,
D.~Bobulska$^{59}$,
J.A.~Boelhauve$^{15}$,
O.~Boente~Garcia$^{46}$,
T.~Boettcher$^{65}$,
A.~Boldyrev$^{82}$,
A.~Bondar$^{43}$,
N.~Bondar$^{38,48}$,
S.~Borghi$^{62}$,
M.~Borisyak$^{42}$,
M.~Borsato$^{17}$,
J.T.~Borsuk$^{35}$,
S.A.~Bouchiba$^{49}$,
T.J.V.~Bowcock$^{60}$,
A.~Boyer$^{48}$,
C.~Bozzi$^{21}$,
M.J.~Bradley$^{61}$,
S.~Braun$^{66}$,
A.~Brea~Rodriguez$^{46}$,
J.~Brodzicka$^{35}$,
A.~Brossa~Gonzalo$^{56}$,
D.~Brundu$^{27}$,
A.~Buonaura$^{50}$,
L.~Buonincontri$^{28}$,
A.T.~Burke$^{62}$,
C.~Burr$^{48}$,
A.~Bursche$^{72}$,
A.~Butkevich$^{39}$,
J.S.~Butter$^{32}$,
J.~Buytaert$^{48}$,
W.~Byczynski$^{48}$,
S.~Cadeddu$^{27}$,
H.~Cai$^{73}$,
R.~Calabrese$^{21,f}$,
L.~Calefice$^{15,13}$,
L.~Calero~Diaz$^{23}$,
S.~Cali$^{23}$,
R.~Calladine$^{53}$,
M.~Calvi$^{26,j}$,
M.~Calvo~Gomez$^{85}$,
P.~Camargo~Magalhaes$^{54}$,
P.~Campana$^{23}$,
A.F.~Campoverde~Quezada$^{6}$,
S.~Capelli$^{26,j}$,
L.~Capriotti$^{20,d}$,
A.~Carbone$^{20,d}$,
G.~Carboni$^{31}$,
R.~Cardinale$^{24,h}$,
A.~Cardini$^{27}$,
I.~Carli$^{4}$,
P.~Carniti$^{26,j}$,
L.~Carus$^{14}$,
K.~Carvalho~Akiba$^{32}$,
A.~Casais~Vidal$^{46}$,
G.~Casse$^{60}$,
M.~Cattaneo$^{48}$,
G.~Cavallero$^{48}$,
S.~Celani$^{49}$,
J.~Cerasoli$^{10}$,
D.~Cervenkov$^{63}$,
A.J.~Chadwick$^{60}$,
M.G.~Chapman$^{54}$,
M.~Charles$^{13}$,
Ph.~Charpentier$^{48}$,
G.~Chatzikonstantinidis$^{53}$,
C.A.~Chavez~Barajas$^{60}$,
M.~Chefdeville$^{8}$,
C.~Chen$^{3}$,
S.~Chen$^{4}$,
A.~Chernov$^{35}$,
V.~Chobanova$^{46}$,
S.~Cholak$^{49}$,
M.~Chrzaszcz$^{35}$,
A.~Chubykin$^{38}$,
V.~Chulikov$^{38}$,
P.~Ciambrone$^{23}$,
M.F.~Cicala$^{56}$,
X.~Cid~Vidal$^{46}$,
G.~Ciezarek$^{48}$,
P.E.L.~Clarke$^{58}$,
M.~Clemencic$^{48}$,
H.V.~Cliff$^{55}$,
J.~Closier$^{48}$,
J.L.~Cobbledick$^{62}$,
V.~Coco$^{48}$,
J.A.B.~Coelho$^{11}$,
J.~Cogan$^{10}$,
E.~Cogneras$^{9}$,
L.~Cojocariu$^{37}$,
P.~Collins$^{48}$,
T.~Colombo$^{48}$,
L.~Congedo$^{19,c}$,
A.~Contu$^{27}$,
N.~Cooke$^{53}$,
G.~Coombs$^{59}$,
I.~Corredoira~$^{46}$,
G.~Corti$^{48}$,
C.M.~Costa~Sobral$^{56}$,
B.~Couturier$^{48}$,
D.C.~Craik$^{64}$,
J.~Crkovsk\'{a}$^{67}$,
M.~Cruz~Torres$^{1}$,
R.~Currie$^{58}$,
C.L.~Da~Silva$^{67}$,
S.~Dadabaev$^{83}$,
L.~Dai$^{71}$,
E.~Dall'Occo$^{15}$,
J.~Dalseno$^{46}$,
C.~D'Ambrosio$^{48}$,
A.~Danilina$^{41}$,
P.~d'Argent$^{48}$,
J.E.~Davies$^{62}$,
A.~Davis$^{62}$,
O.~De~Aguiar~Francisco$^{62}$,
K.~De~Bruyn$^{79}$,
S.~De~Capua$^{62}$,
M.~De~Cian$^{49}$,
J.M.~De~Miranda$^{1}$,
L.~De~Paula$^{2}$,
M.~De~Serio$^{19,c}$,
D.~De~Simone$^{50}$,
P.~De~Simone$^{23}$,
F.~De~Vellis$^{15}$,
J.A.~de~Vries$^{80}$,
C.T.~Dean$^{67}$,
F.~Debernardis$^{19,c}$,
D.~Decamp$^{8}$,
V.~Dedu$^{10}$,
L.~Del~Buono$^{13}$,
B.~Delaney$^{55}$,
H.-P.~Dembinski$^{15}$,
A.~Dendek$^{34}$,
V.~Denysenko$^{50}$,
D.~Derkach$^{82}$,
O.~Deschamps$^{9}$,
F.~Desse$^{11}$,
F.~Dettori$^{27,e}$,
B.~Dey$^{77}$,
A.~Di~Cicco$^{23}$,
P.~Di~Nezza$^{23}$,
S.~Didenko$^{83}$,
L.~Dieste~Maronas$^{46}$,
H.~Dijkstra$^{48}$,
V.~Dobishuk$^{52}$,
C.~Dong$^{3}$,
A.M.~Donohoe$^{18}$,
F.~Dordei$^{27}$,
A.C.~dos~Reis$^{1}$,
L.~Douglas$^{59}$,
A.~Dovbnya$^{51}$,
A.G.~Downes$^{8}$,
M.W.~Dudek$^{35}$,
L.~Dufour$^{48}$,
V.~Duk$^{78}$,
P.~Durante$^{48}$,
J.M.~Durham$^{67}$,
D.~Dutta$^{62}$,
A.~Dziurda$^{35}$,
A.~Dzyuba$^{38}$,
S.~Easo$^{57}$,
U.~Egede$^{69}$,
V.~Egorychev$^{41}$,
S.~Eidelman$^{43,u,\dagger}$,
S.~Eisenhardt$^{58}$,
S.~Ek-In$^{49}$,
L.~Eklund$^{59,86}$,
S.~Ely$^{68}$,
A.~Ene$^{37}$,
E.~Epple$^{67}$,
S.~Escher$^{14}$,
J.~Eschle$^{50}$,
S.~Esen$^{13}$,
T.~Evans$^{48}$,
A.~Falabella$^{20}$,
J.~Fan$^{3}$,
Y.~Fan$^{6}$,
B.~Fang$^{73}$,
S.~Farry$^{60}$,
D.~Fazzini$^{26,j}$,
M.~F{\'e}o$^{48}$,
A.~Fernandez~Prieto$^{46}$,
A.D.~Fernez$^{66}$,
F.~Ferrari$^{20,d}$,
L.~Ferreira~Lopes$^{49}$,
F.~Ferreira~Rodrigues$^{2}$,
S.~Ferreres~Sole$^{32}$,
M.~Ferrillo$^{50}$,
M.~Ferro-Luzzi$^{48}$,
S.~Filippov$^{39}$,
R.A.~Fini$^{19}$,
M.~Fiorini$^{21,f}$,
M.~Firlej$^{34}$,
K.M.~Fischer$^{63}$,
D.S.~Fitzgerald$^{87}$,
C.~Fitzpatrick$^{62}$,
T.~Fiutowski$^{34}$,
A.~Fkiaras$^{48}$,
F.~Fleuret$^{12}$,
M.~Fontana$^{13}$,
F.~Fontanelli$^{24,h}$,
R.~Forty$^{48}$,
D.~Foulds-Holt$^{55}$,
V.~Franco~Lima$^{60}$,
M.~Franco~Sevilla$^{66}$,
M.~Frank$^{48}$,
E.~Franzoso$^{21}$,
G.~Frau$^{17}$,
C.~Frei$^{48}$,
D.A.~Friday$^{59}$,
J.~Fu$^{6}$,
Q.~Fuehring$^{15}$,
E.~Gabriel$^{32}$,
G.~Galati$^{19,c}$,
A.~Gallas~Torreira$^{46}$,
D.~Galli$^{20,d}$,
S.~Gambetta$^{58,48}$,
Y.~Gan$^{3}$,
M.~Gandelman$^{2}$,
P.~Gandini$^{25}$,
Y.~Gao$^{5}$,
M.~Garau$^{27}$,
L.M.~Garcia~Martin$^{56}$,
P.~Garcia~Moreno$^{45}$,
J.~Garc{\'\i}a~Pardi{\~n}as$^{26,j}$,
B.~Garcia~Plana$^{46}$,
F.A.~Garcia~Rosales$^{12}$,
L.~Garrido$^{45}$,
C.~Gaspar$^{48}$,
R.E.~Geertsema$^{32}$,
D.~Gerick$^{17}$,
L.L.~Gerken$^{15}$,
E.~Gersabeck$^{62}$,
M.~Gersabeck$^{62}$,
T.~Gershon$^{56}$,
D.~Gerstel$^{10}$,
L.~Giambastiani$^{28}$,
V.~Gibson$^{55}$,
H.K.~Giemza$^{36}$,
A.L.~Gilman$^{63}$,
M.~Giovannetti$^{23,p}$,
A.~Giovent{\`u}$^{46}$,
P.~Gironella~Gironell$^{45}$,
L.~Giubega$^{37}$,
C.~Giugliano$^{21,f,48}$,
K.~Gizdov$^{58}$,
E.L.~Gkougkousis$^{48}$,
V.V.~Gligorov$^{13}$,
C.~G{\"o}bel$^{70}$,
E.~Golobardes$^{85}$,
D.~Golubkov$^{41}$,
A.~Golutvin$^{61,83}$,
A.~Gomes$^{1,a}$,
S.~Gomez~Fernandez$^{45}$,
F.~Goncalves~Abrantes$^{63}$,
M.~Goncerz$^{35}$,
G.~Gong$^{3}$,
P.~Gorbounov$^{41}$,
I.V.~Gorelov$^{40}$,
C.~Gotti$^{26}$,
E.~Govorkova$^{48}$,
J.P.~Grabowski$^{17}$,
T.~Grammatico$^{13}$,
L.A.~Granado~Cardoso$^{48}$,
E.~Graug{\'e}s$^{45}$,
E.~Graverini$^{49}$,
G.~Graziani$^{22}$,
A.~Grecu$^{37}$,
L.M.~Greeven$^{32}$,
N.A.~Grieser$^{4}$,
L.~Grillo$^{62}$,
S.~Gromov$^{83}$,
B.R.~Gruberg~Cazon$^{63}$,
C.~Gu$^{3}$,
M.~Guarise$^{21}$,
M.~Guittiere$^{11}$,
P. A.~G{\"u}nther$^{17}$,
E.~Gushchin$^{39}$,
A.~Guth$^{14}$,
Y.~Guz$^{44}$,
T.~Gys$^{48}$,
T.~Hadavizadeh$^{69}$,
G.~Haefeli$^{49}$,
C.~Haen$^{48}$,
J.~Haimberger$^{48}$,
T.~Halewood-leagas$^{60}$,
P.M.~Hamilton$^{66}$,
J.P.~Hammerich$^{60}$,
Q.~Han$^{7}$,
X.~Han$^{17}$,
T.H.~Hancock$^{63}$,
E.B.~Hansen$^{62}$,
S.~Hansmann-Menzemer$^{17}$,
N.~Harnew$^{63}$,
T.~Harrison$^{60}$,
C.~Hasse$^{48}$,
M.~Hatch$^{48}$,
J.~He$^{6,b}$,
M.~Hecker$^{61}$,
K.~Heijhoff$^{32}$,
K.~Heinicke$^{15}$,
A.M.~Hennequin$^{48}$,
K.~Hennessy$^{60}$,
L.~Henry$^{48}$,
J.~Heuel$^{14}$,
A.~Hicheur$^{2}$,
D.~Hill$^{49}$,
M.~Hilton$^{62}$,
S.E.~Hollitt$^{15}$,
R.~Hou$^{7}$,
Y.~Hou$^{8}$,
J.~Hu$^{17}$,
J.~Hu$^{72}$,
W.~Hu$^{7}$,
X.~Hu$^{3}$,
W.~Huang$^{6}$,
X.~Huang$^{73}$,
W.~Hulsbergen$^{32}$,
R.J.~Hunter$^{56}$,
M.~Hushchyn$^{82}$,
D.~Hutchcroft$^{60}$,
D.~Hynds$^{32}$,
P.~Ibis$^{15}$,
M.~Idzik$^{34}$,
D.~Ilin$^{38}$,
P.~Ilten$^{65}$,
A.~Inglessi$^{38}$,
A.~Ishteev$^{83}$,
K.~Ivshin$^{38}$,
R.~Jacobsson$^{48}$,
H.~Jage$^{14}$,
S.~Jakobsen$^{48}$,
E.~Jans$^{32}$,
B.K.~Jashal$^{47}$,
A.~Jawahery$^{66}$,
V.~Jevtic$^{15}$,
F.~Jiang$^{3}$,
M.~John$^{63}$,
D.~Johnson$^{48}$,
C.R.~Jones$^{55}$,
T.P.~Jones$^{56}$,
B.~Jost$^{48}$,
N.~Jurik$^{48}$,
S.H.~Kalavan~Kadavath$^{34}$,
S.~Kandybei$^{51}$,
Y.~Kang$^{3}$,
M.~Karacson$^{48}$,
M.~Karpov$^{82}$,
F.~Keizer$^{48}$,
D.M.~Keller$^{68}$,
M.~Kenzie$^{56}$,
T.~Ketel$^{33}$,
B.~Khanji$^{15}$,
A.~Kharisova$^{84}$,
S.~Kholodenko$^{44}$,
T.~Kirn$^{14}$,
V.S.~Kirsebom$^{49}$,
O.~Kitouni$^{64}$,
S.~Klaver$^{32}$,
N.~Kleijne$^{29}$,
K.~Klimaszewski$^{36}$,
M.R.~Kmiec$^{36}$,
S.~Koliiev$^{52}$,
A.~Kondybayeva$^{83}$,
A.~Konoplyannikov$^{41}$,
P.~Kopciewicz$^{34}$,
R.~Kopecna$^{17}$,
P.~Koppenburg$^{32}$,
M.~Korolev$^{40}$,
I.~Kostiuk$^{32,52}$,
O.~Kot$^{52}$,
S.~Kotriakhova$^{21,38}$,
P.~Kravchenko$^{38}$,
L.~Kravchuk$^{39}$,
R.D.~Krawczyk$^{48}$,
M.~Kreps$^{56}$,
F.~Kress$^{61}$,
S.~Kretzschmar$^{14}$,
P.~Krokovny$^{43,u}$,
W.~Krupa$^{34}$,
W.~Krzemien$^{36}$,
M.~Kucharczyk$^{35}$,
V.~Kudryavtsev$^{43,u}$,
H.S.~Kuindersma$^{32,33}$,
G.J.~Kunde$^{67}$,
T.~Kvaratskheliya$^{41}$,
D.~Lacarrere$^{48}$,
G.~Lafferty$^{62}$,
A.~Lai$^{27}$,
A.~Lampis$^{27}$,
D.~Lancierini$^{50}$,
J.J.~Lane$^{62}$,
R.~Lane$^{54}$,
G.~Lanfranchi$^{23}$,
C.~Langenbruch$^{14}$,
J.~Langer$^{15}$,
O.~Lantwin$^{83}$,
T.~Latham$^{56}$,
F.~Lazzari$^{29,q}$,
R.~Le~Gac$^{10}$,
S.H.~Lee$^{87}$,
R.~Lef{\`e}vre$^{9}$,
A.~Leflat$^{40}$,
S.~Legotin$^{83}$,
O.~Leroy$^{10}$,
T.~Lesiak$^{35}$,
B.~Leverington$^{17}$,
H.~Li$^{72}$,
P.~Li$^{17}$,
S.~Li$^{7}$,
Y.~Li$^{4}$,
Y.~Li$^{4}$,
Z.~Li$^{68}$,
X.~Liang$^{68}$,
T.~Lin$^{61}$,
R.~Lindner$^{48}$,
V.~Lisovskyi$^{15}$,
R.~Litvinov$^{27}$,
G.~Liu$^{72}$,
H.~Liu$^{6}$,
Q.~Liu$^{6}$,
S.~Liu$^{4}$,
A.~Lobo~Salvia$^{45}$,
A.~Loi$^{27}$,
J.~Lomba~Castro$^{46}$,
I.~Longstaff$^{59}$,
J.H.~Lopes$^{2}$,
S.~Lopez~Solino$^{46}$,
G.H.~Lovell$^{55}$,
Y.~Lu$^{4}$,
C.~Lucarelli$^{22,g}$,
D.~Lucchesi$^{28,l}$,
S.~Luchuk$^{39}$,
M.~Lucio~Martinez$^{32}$,
V.~Lukashenko$^{32,52}$,
Y.~Luo$^{3}$,
A.~Lupato$^{62}$,
E.~Luppi$^{21,f}$,
O.~Lupton$^{56}$,
A.~Lusiani$^{29,m}$,
X.~Lyu$^{6}$,
L.~Ma$^{4}$,
R.~Ma$^{6}$,
S.~Maccolini$^{20,d}$,
F.~Machefert$^{11}$,
F.~Maciuc$^{37}$,
V.~Macko$^{49}$,
P.~Mackowiak$^{15}$,
S.~Maddrell-Mander$^{54}$,
O.~Madejczyk$^{34}$,
L.R.~Madhan~Mohan$^{54}$,
O.~Maev$^{38}$,
A.~Maevskiy$^{82}$,
D.~Maisuzenko$^{38}$,
M.W.~Majewski$^{34}$,
J.J.~Malczewski$^{35}$,
S.~Malde$^{63}$,
B.~Malecki$^{48}$,
A.~Malinin$^{81}$,
T.~Maltsev$^{43,u}$,
H.~Malygina$^{17}$,
G.~Manca$^{27,e}$,
G.~Mancinelli$^{10}$,
D.~Manuzzi$^{20,d}$,
D.~Marangotto$^{25,i}$,
J.~Maratas$^{9,s}$,
J.F.~Marchand$^{8}$,
U.~Marconi$^{20}$,
S.~Mariani$^{22,g}$,
C.~Marin~Benito$^{48}$,
M.~Marinangeli$^{49}$,
J.~Marks$^{17}$,
A.M.~Marshall$^{54}$,
P.J.~Marshall$^{60}$,
G.~Martelli$^{78}$,
G.~Martellotti$^{30}$,
L.~Martinazzoli$^{48,j}$,
M.~Martinelli$^{26,j}$,
D.~Martinez~Santos$^{46}$,
F.~Martinez~Vidal$^{47}$,
A.~Massafferri$^{1}$,
M.~Materok$^{14}$,
R.~Matev$^{48}$,
A.~Mathad$^{50}$,
V.~Matiunin$^{41}$,
C.~Matteuzzi$^{26}$,
K.R.~Mattioli$^{87}$,
A.~Mauri$^{32}$,
E.~Maurice$^{12}$,
J.~Mauricio$^{45}$,
M.~Mazurek$^{48}$,
M.~McCann$^{61}$,
L.~Mcconnell$^{18}$,
T.H.~Mcgrath$^{62}$,
N.T.~Mchugh$^{59}$,
A.~McNab$^{62}$,
R.~McNulty$^{18}$,
J.V.~Mead$^{60}$,
B.~Meadows$^{65}$,
G.~Meier$^{15}$,
N.~Meinert$^{76}$,
D.~Melnychuk$^{36}$,
S.~Meloni$^{26,j}$,
M.~Merk$^{32,80}$,
A.~Merli$^{25}$,
L.~Meyer~Garcia$^{2}$,
M.~Mikhasenko$^{48}$,
D.A.~Milanes$^{74}$,
E.~Millard$^{56}$,
M.~Milovanovic$^{48}$,
M.-N.~Minard$^{8}$,
A.~Minotti$^{26,j}$,
L.~Minzoni$^{21,f}$,
S.E.~Mitchell$^{58}$,
B.~Mitreska$^{62}$,
D.S.~Mitzel$^{15}$,
A.~M{\"o}dden~$^{15}$,
R.A.~Mohammed$^{63}$,
R.D.~Moise$^{61}$,
S.~Mokhnenko$^{82}$,
T.~Momb{\"a}cher$^{46}$,
I.A.~Monroy$^{74}$,
S.~Monteil$^{9}$,
M.~Morandin$^{28}$,
G.~Morello$^{23}$,
M.J.~Morello$^{29,m}$,
J.~Moron$^{34}$,
A.B.~Morris$^{75}$,
A.G.~Morris$^{56}$,
R.~Mountain$^{68}$,
H.~Mu$^{3}$,
F.~Muheim$^{58,48}$,
M.~Mulder$^{48}$,
D.~M{\"u}ller$^{48}$,
K.~M{\"u}ller$^{50}$,
C.H.~Murphy$^{63}$,
D.~Murray$^{62}$,
P.~Muzzetto$^{27,48}$,
P.~Naik$^{54}$,
T.~Nakada$^{49}$,
R.~Nandakumar$^{57}$,
T.~Nanut$^{49}$,
I.~Nasteva$^{2}$,
M.~Needham$^{58}$,
I.~Neri$^{21}$,
N.~Neri$^{25,i}$,
S.~Neubert$^{75}$,
N.~Neufeld$^{48}$,
R.~Newcombe$^{61}$,
E.M.~Niel$^{11}$,
S.~Nieswand$^{14}$,
N.~Nikitin$^{40}$,
N.S.~Nolte$^{64}$,
C.~Normand$^{8}$,
C.~Nunez$^{87}$,
A.~Oblakowska-Mucha$^{34}$,
V.~Obraztsov$^{44}$,
T.~Oeser$^{14}$,
D.P.~O'Hanlon$^{54}$,
S.~Okamura$^{21}$,
R.~Oldeman$^{27,e}$,
F.~Oliva$^{58}$,
M.E.~Olivares$^{68}$,
C.J.G.~Onderwater$^{79}$,
R.H.~O'neil$^{58}$,
J.M.~Otalora~Goicochea$^{2}$,
T.~Ovsiannikova$^{41}$,
P.~Owen$^{50}$,
A.~Oyanguren$^{47}$,
K.O.~Padeken$^{75}$,
B.~Pagare$^{56}$,
P.R.~Pais$^{48}$,
T.~Pajero$^{63}$,
A.~Palano$^{19}$,
M.~Palutan$^{23}$,
Y.~Pan$^{62}$,
G.~Panshin$^{84}$,
A.~Papanestis$^{57}$,
M.~Pappagallo$^{19,c}$,
L.L.~Pappalardo$^{21,f}$,
C.~Pappenheimer$^{65}$,
W.~Parker$^{66}$,
C.~Parkes$^{62}$,
B.~Passalacqua$^{21}$,
G.~Passaleva$^{22}$,
A.~Pastore$^{19}$,
M.~Patel$^{61}$,
C.~Patrignani$^{20,d}$,
C.J.~Pawley$^{80}$,
A.~Pearce$^{48}$,
A.~Pellegrino$^{32}$,
M.~Pepe~Altarelli$^{48}$,
S.~Perazzini$^{20}$,
D.~Pereima$^{41}$,
A.~Pereiro~Castro$^{46}$,
P.~Perret$^{9}$,
M.~Petric$^{59,48}$,
K.~Petridis$^{54}$,
A.~Petrolini$^{24,h}$,
A.~Petrov$^{81}$,
S.~Petrucci$^{58}$,
M.~Petruzzo$^{25}$,
T.T.H.~Pham$^{68}$,
L.~Pica$^{29,m}$,
M.~Piccini$^{78}$,
B.~Pietrzyk$^{8}$,
G.~Pietrzyk$^{49}$,
M.~Pili$^{63}$,
D.~Pinci$^{30}$,
F.~Pisani$^{48}$,
M.~Pizzichemi$^{26,48,j}$,
Resmi ~P.K$^{10}$,
V.~Placinta$^{37}$,
J.~Plews$^{53}$,
M.~Plo~Casasus$^{46}$,
F.~Polci$^{13}$,
M.~Poli~Lener$^{23}$,
M.~Poliakova$^{68}$,
A.~Poluektov$^{10}$,
N.~Polukhina$^{83,t}$,
I.~Polyakov$^{68}$,
E.~Polycarpo$^{2}$,
S.~Ponce$^{48}$,
D.~Popov$^{6,48}$,
S.~Popov$^{42}$,
S.~Poslavskii$^{44}$,
K.~Prasanth$^{35}$,
L.~Promberger$^{48}$,
C.~Prouve$^{46}$,
V.~Pugatch$^{52}$,
V.~Puill$^{11}$,
H.~Pullen$^{63}$,
G.~Punzi$^{29,n}$,
H.~Qi$^{3}$,
W.~Qian$^{6}$,
J.~Qin$^{6}$,
N.~Qin$^{3}$,
R.~Quagliani$^{49}$,
B.~Quintana$^{8}$,
N.V.~Raab$^{18}$,
R.I.~Rabadan~Trejo$^{6}$,
B.~Rachwal$^{34}$,
J.H.~Rademacker$^{54}$,
M.~Rama$^{29}$,
M.~Ramos~Pernas$^{56}$,
M.S.~Rangel$^{2}$,
F.~Ratnikov$^{42,82}$,
G.~Raven$^{33}$,
M.~Reboud$^{8}$,
F.~Redi$^{49}$,
F.~Reiss$^{62}$,
C.~Remon~Alepuz$^{47}$,
Z.~Ren$^{3}$,
V.~Renaudin$^{63}$,
R.~Ribatti$^{29}$,
S.~Ricciardi$^{57}$,
K.~Rinnert$^{60}$,
P.~Robbe$^{11}$,
G.~Robertson$^{58}$,
A.B.~Rodrigues$^{49}$,
E.~Rodrigues$^{60}$,
J.A.~Rodriguez~Lopez$^{74}$,
E.R.R.~Rodriguez~Rodriguez$^{46}$,
A.~Rollings$^{63}$,
P.~Roloff$^{48}$,
V.~Romanovskiy$^{44}$,
M.~Romero~Lamas$^{46}$,
A.~Romero~Vidal$^{46}$,
J.D.~Roth$^{87}$,
M.~Rotondo$^{23}$,
M.S.~Rudolph$^{68}$,
T.~Ruf$^{48}$,
R.A.~Ruiz~Fernandez$^{46}$,
J.~Ruiz~Vidal$^{47}$,
A.~Ryzhikov$^{82}$,
J.~Ryzka$^{34}$,
J.J.~Saborido~Silva$^{46}$,
N.~Sagidova$^{38}$,
N.~Sahoo$^{56}$,
B.~Saitta$^{27,e}$,
M.~Salomoni$^{48}$,
C.~Sanchez~Gras$^{32}$,
R.~Santacesaria$^{30}$,
C.~Santamarina~Rios$^{46}$,
M.~Santimaria$^{23}$,
E.~Santovetti$^{31,p}$,
D.~Saranin$^{83}$,
G.~Sarpis$^{14}$,
M.~Sarpis$^{75}$,
A.~Sarti$^{30}$,
C.~Satriano$^{30,o}$,
A.~Satta$^{31}$,
M.~Saur$^{15}$,
D.~Savrina$^{41,40}$,
H.~Sazak$^{9}$,
L.G.~Scantlebury~Smead$^{63}$,
A.~Scarabotto$^{13}$,
S.~Schael$^{14}$,
S.~Scherl$^{60}$,
M.~Schiller$^{59}$,
H.~Schindler$^{48}$,
M.~Schmelling$^{16}$,
B.~Schmidt$^{48}$,
S.~Schmitt$^{14}$,
O.~Schneider$^{49}$,
A.~Schopper$^{48}$,
M.~Schubiger$^{32}$,
S.~Schulte$^{49}$,
M.H.~Schune$^{11}$,
R.~Schwemmer$^{48}$,
B.~Sciascia$^{23,48}$,
S.~Sellam$^{46}$,
A.~Semennikov$^{41}$,
M.~Senghi~Soares$^{33}$,
A.~Sergi$^{24,h}$,
N.~Serra$^{50}$,
L.~Sestini$^{28}$,
A.~Seuthe$^{15}$,
Y.~Shang$^{5}$,
D.M.~Shangase$^{87}$,
M.~Shapkin$^{44}$,
I.~Shchemerov$^{83}$,
L.~Shchutska$^{49}$,
T.~Shears$^{60}$,
L.~Shekhtman$^{43,u}$,
Z.~Shen$^{5}$,
V.~Shevchenko$^{81}$,
E.B.~Shields$^{26,j}$,
Y.~Shimizu$^{11}$,
E.~Shmanin$^{83}$,
J.D.~Shupperd$^{68}$,
B.G.~Siddi$^{21}$,
R.~Silva~Coutinho$^{50}$,
G.~Simi$^{28}$,
S.~Simone$^{19,c}$,
N.~Skidmore$^{62}$,
T.~Skwarnicki$^{68}$,
M.W.~Slater$^{53}$,
I.~Slazyk$^{21,f}$,
J.C.~Smallwood$^{63}$,
J.G.~Smeaton$^{55}$,
A.~Smetkina$^{41}$,
E.~Smith$^{50}$,
M.~Smith$^{61}$,
A.~Snoch$^{32}$,
M.~Soares$^{20}$,
L.~Soares~Lavra$^{9}$,
M.D.~Sokoloff$^{65}$,
F.J.P.~Soler$^{59}$,
A.~Solovev$^{38}$,
I.~Solovyev$^{38}$,
F.L.~Souza~De~Almeida$^{2}$,
B.~Souza~De~Paula$^{2}$,
B.~Spaan$^{15}$,
E.~Spadaro~Norella$^{25}$,
P.~Spradlin$^{59}$,
F.~Stagni$^{48}$,
M.~Stahl$^{65}$,
S.~Stahl$^{48}$,
S.~Stanislaus$^{63}$,
O.~Steinkamp$^{50,83}$,
O.~Stenyakin$^{44}$,
H.~Stevens$^{15}$,
S.~Stone$^{68}$,
M.~Straticiuc$^{37}$,
D.~Strekalina$^{83}$,
F.~Suljik$^{63}$,
J.~Sun$^{27}$,
L.~Sun$^{73}$,
Y.~Sun$^{66}$,
P.~Svihra$^{62}$,
P.N.~Swallow$^{53}$,
K.~Swientek$^{34}$,
A.~Szabelski$^{36}$,
T.~Szumlak$^{34}$,
M.~Szymanski$^{48}$,
S.~Taneja$^{62}$,
A.R.~Tanner$^{54}$,
M.D.~Tat$^{63}$,
A.~Terentev$^{83}$,
F.~Teubert$^{48}$,
E.~Thomas$^{48}$,
D.J.D.~Thompson$^{53}$,
K.A.~Thomson$^{60}$,
V.~Tisserand$^{9}$,
S.~T'Jampens$^{8}$,
M.~Tobin$^{4}$,
L.~Tomassetti$^{21,f}$,
X.~Tong$^{5}$,
D.~Torres~Machado$^{1}$,
D.Y.~Tou$^{13}$,
E.~Trifonova$^{83}$,
C.~Trippl$^{49}$,
G.~Tuci$^{6}$,
A.~Tully$^{49}$,
N.~Tuning$^{32,48}$,
A.~Ukleja$^{36}$,
D.J.~Unverzagt$^{17}$,
E.~Ursov$^{83}$,
A.~Usachov$^{32}$,
A.~Ustyuzhanin$^{42,82}$,
U.~Uwer$^{17}$,
A.~Vagner$^{84}$,
V.~Vagnoni$^{20}$,
A.~Valassi$^{48}$,
G.~Valenti$^{20}$,
N.~Valls~Canudas$^{85}$,
M.~van~Beuzekom$^{32}$,
M.~Van~Dijk$^{49}$,
E.~van~Herwijnen$^{83}$,
C.B.~Van~Hulse$^{18}$,
M.~van~Veghel$^{79}$,
R.~Vazquez~Gomez$^{45}$,
P.~Vazquez~Regueiro$^{46}$,
C.~V{\'a}zquez~Sierra$^{48}$,
S.~Vecchi$^{21}$,
J.J.~Velthuis$^{54}$,
M.~Veltri$^{22,r}$,
A.~Venkateswaran$^{68}$,
M.~Veronesi$^{32}$,
M.~Vesterinen$^{56}$,
D.~~Vieira$^{65}$,
M.~Vieites~Diaz$^{49}$,
H.~Viemann$^{76}$,
X.~Vilasis-Cardona$^{85}$,
E.~Vilella~Figueras$^{60}$,
A.~Villa$^{20}$,
P.~Vincent$^{13}$,
F.C.~Volle$^{11}$,
D.~Vom~Bruch$^{10}$,
A.~Vorobyev$^{38}$,
V.~Vorobyev$^{43,u}$,
N.~Voropaev$^{38}$,
K.~Vos$^{80}$,
R.~Waldi$^{17}$,
J.~Walsh$^{29}$,
C.~Wang$^{17}$,
J.~Wang$^{5}$,
J.~Wang$^{4}$,
J.~Wang$^{3}$,
J.~Wang$^{73}$,
M.~Wang$^{3}$,
R.~Wang$^{54}$,
Y.~Wang$^{7}$,
Z.~Wang$^{50}$,
Z.~Wang$^{3}$,
Z.~Wang$^{6}$,
J.A.~Ward$^{56}$,
N.K.~Watson$^{53}$,
S.G.~Weber$^{13}$,
D.~Websdale$^{61}$,
C.~Weisser$^{64}$,
B.D.C.~Westhenry$^{54}$,
D.J.~White$^{62}$,
M.~Whitehead$^{54}$,
A.R.~Wiederhold$^{56}$,
D.~Wiedner$^{15}$,
G.~Wilkinson$^{63}$,
M.~Wilkinson$^{68}$,
I.~Williams$^{55}$,
M.~Williams$^{64}$,
M.R.J.~Williams$^{58}$,
F.F.~Wilson$^{57}$,
W.~Wislicki$^{36}$,
M.~Witek$^{35}$,
L.~Witola$^{17}$,
G.~Wormser$^{11}$,
S.A.~Wotton$^{55}$,
H.~Wu$^{68}$,
K.~Wyllie$^{48}$,
Z.~Xiang$^{6}$,
D.~Xiao$^{7}$,
Y.~Xie$^{7}$,
A.~Xu$^{5}$,
J.~Xu$^{6}$,
L.~Xu$^{3}$,
M.~Xu$^{7}$,
Q.~Xu$^{6}$,
Z.~Xu$^{5}$,
Z.~Xu$^{6}$,
D.~Yang$^{3}$,
S.~Yang$^{6}$,
Y.~Yang$^{6}$,
Z.~Yang$^{5}$,
Z.~Yang$^{66}$,
Y.~Yao$^{68}$,
L.E.~Yeomans$^{60}$,
H.~Yin$^{7}$,
J.~Yu$^{71}$,
X.~Yuan$^{68}$,
O.~Yushchenko$^{44}$,
E.~Zaffaroni$^{49}$,
M.~Zavertyaev$^{16,t}$,
M.~Zdybal$^{35}$,
O.~Zenaiev$^{48}$,
M.~Zeng$^{3}$,
D.~Zhang$^{7}$,
L.~Zhang$^{3}$,
S.~Zhang$^{71}$,
S.~Zhang$^{5}$,
Y.~Zhang$^{5}$,
Y.~Zhang$^{63}$,
A.~Zharkova$^{83}$,
A.~Zhelezov$^{17}$,
Y.~Zheng$^{6}$,
T.~Zhou$^{5}$,
X.~Zhou$^{6}$,
Y.~Zhou$^{6}$,
V.~Zhovkovska$^{11}$,
X.~Zhu$^{3}$,
X.~Zhu$^{7}$,
Z.~Zhu$^{6}$,
V.~Zhukov$^{14,40}$,
J.B.~Zonneveld$^{58}$,
Q.~Zou$^{4}$,
S.~Zucchelli$^{20,d}$,
D.~Zuliani$^{28}$,
G.~Zunica$^{62}$.\bigskip

{\footnotesize \it

$^{1}$Centro Brasileiro de Pesquisas F{\'\i}sicas (CBPF), Rio de Janeiro, Brazil\\
$^{2}$Universidade Federal do Rio de Janeiro (UFRJ), Rio de Janeiro, Brazil\\
$^{3}$Center for High Energy Physics, Tsinghua University, Beijing, China\\
$^{4}$Institute Of High Energy Physics (IHEP), Beijing, China\\
$^{5}$School of Physics State Key Laboratory of Nuclear Physics and Technology, Peking University, Beijing, China\\
$^{6}$University of Chinese Academy of Sciences, Beijing, China\\
$^{7}$Institute of Particle Physics, Central China Normal University, Wuhan, Hubei, China\\
$^{8}$Univ. Savoie Mont Blanc, CNRS, IN2P3-LAPP, Annecy, France\\
$^{9}$Universit{\'e} Clermont Auvergne, CNRS/IN2P3, LPC, Clermont-Ferrand, France\\
$^{10}$Aix Marseille Univ, CNRS/IN2P3, CPPM, Marseille, France\\
$^{11}$Universit{\'e} Paris-Saclay, CNRS/IN2P3, IJCLab, Orsay, France\\
$^{12}$Laboratoire Leprince-Ringuet, CNRS/IN2P3, Ecole Polytechnique, Institut Polytechnique de Paris, Palaiseau, France\\
$^{13}$LPNHE, Sorbonne Universit{\'e}, Paris Diderot Sorbonne Paris Cit{\'e}, CNRS/IN2P3, Paris, France\\
$^{14}$I. Physikalisches Institut, RWTH Aachen University, Aachen, Germany\\
$^{15}$Fakult{\"a}t Physik, Technische Universit{\"a}t Dortmund, Dortmund, Germany\\
$^{16}$Max-Planck-Institut f{\"u}r Kernphysik (MPIK), Heidelberg, Germany\\
$^{17}$Physikalisches Institut, Ruprecht-Karls-Universit{\"a}t Heidelberg, Heidelberg, Germany\\
$^{18}$School of Physics, University College Dublin, Dublin, Ireland\\
$^{19}$INFN Sezione di Bari, Bari, Italy\\
$^{20}$INFN Sezione di Bologna, Bologna, Italy\\
$^{21}$INFN Sezione di Ferrara, Ferrara, Italy\\
$^{22}$INFN Sezione di Firenze, Firenze, Italy\\
$^{23}$INFN Laboratori Nazionali di Frascati, Frascati, Italy\\
$^{24}$INFN Sezione di Genova, Genova, Italy\\
$^{25}$INFN Sezione di Milano, Milano, Italy\\
$^{26}$INFN Sezione di Milano-Bicocca, Milano, Italy\\
$^{27}$INFN Sezione di Cagliari, Monserrato, Italy\\
$^{28}$Universita degli Studi di Padova, Universita e INFN, Padova, Padova, Italy\\
$^{29}$INFN Sezione di Pisa, Pisa, Italy\\
$^{30}$INFN Sezione di Roma La Sapienza, Roma, Italy\\
$^{31}$INFN Sezione di Roma Tor Vergata, Roma, Italy\\
$^{32}$Nikhef National Institute for Subatomic Physics, Amsterdam, Netherlands\\
$^{33}$Nikhef National Institute for Subatomic Physics and VU University Amsterdam, Amsterdam, Netherlands\\
$^{34}$AGH - University of Science and Technology, Faculty of Physics and Applied Computer Science, Krak{\'o}w, Poland\\
$^{35}$Henryk Niewodniczanski Institute of Nuclear Physics  Polish Academy of Sciences, Krak{\'o}w, Poland\\
$^{36}$National Center for Nuclear Research (NCBJ), Warsaw, Poland\\
$^{37}$Horia Hulubei National Institute of Physics and Nuclear Engineering, Bucharest-Magurele, Romania\\
$^{38}$Petersburg Nuclear Physics Institute NRC Kurchatov Institute (PNPI NRC KI), Gatchina, Russia\\
$^{39}$Institute for Nuclear Research of the Russian Academy of Sciences (INR RAS), Moscow, Russia\\
$^{40}$Institute of Nuclear Physics, Moscow State University (SINP MSU), Moscow, Russia\\
$^{41}$Institute of Theoretical and Experimental Physics NRC Kurchatov Institute (ITEP NRC KI), Moscow, Russia\\
$^{42}$Yandex School of Data Analysis, Moscow, Russia\\
$^{43}$Budker Institute of Nuclear Physics (SB RAS), Novosibirsk, Russia\\
$^{44}$Institute for High Energy Physics NRC Kurchatov Institute (IHEP NRC KI), Protvino, Russia, Protvino, Russia\\
$^{45}$ICCUB, Universitat de Barcelona, Barcelona, Spain\\
$^{46}$Instituto Galego de F{\'\i}sica de Altas Enerx{\'\i}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain\\
$^{47}$Instituto de Fisica Corpuscular, Centro Mixto Universidad de Valencia - CSIC, Valencia, Spain\\
$^{48}$European Organization for Nuclear Research (CERN), Geneva, Switzerland\\
$^{49}$Institute of Physics, Ecole Polytechnique  F{\'e}d{\'e}rale de Lausanne (EPFL), Lausanne, Switzerland\\
$^{50}$Physik-Institut, Universit{\"a}t Z{\"u}rich, Z{\"u}rich, Switzerland\\
$^{51}$NSC Kharkiv Institute of Physics and Technology (NSC KIPT), Kharkiv, Ukraine\\
$^{52}$Institute for Nuclear Research of the National Academy of Sciences (KINR), Kyiv, Ukraine\\
$^{53}$University of Birmingham, Birmingham, United Kingdom\\
$^{54}$H.H. Wills Physics Laboratory, University of Bristol, Bristol, United Kingdom\\
$^{55}$Cavendish Laboratory, University of Cambridge, Cambridge, United Kingdom\\
$^{56}$Department of Physics, University of Warwick, Coventry, United Kingdom\\
$^{57}$STFC Rutherford Appleton Laboratory, Didcot, United Kingdom\\
$^{58}$School of Physics and Astronomy, University of Edinburgh, Edinburgh, United Kingdom\\
$^{59}$School of Physics and Astronomy, University of Glasgow, Glasgow, United Kingdom\\
$^{60}$Oliver Lodge Laboratory, University of Liverpool, Liverpool, United Kingdom\\
$^{61}$Imperial College London, London, United Kingdom\\
$^{62}$Department of Physics and Astronomy, University of Manchester, Manchester, United Kingdom\\
$^{63}$Department of Physics, University of Oxford, Oxford, United Kingdom\\
$^{64}$Massachusetts Institute of Technology, Cambridge, MA, United States\\
$^{65}$University of Cincinnati, Cincinnati, OH, United States\\
$^{66}$University of Maryland, College Park, MD, United States\\
$^{67}$Los Alamos National Laboratory (LANL), Los Alamos, United States\\
$^{68}$Syracuse University, Syracuse, NY, United States\\
$^{69}$School of Physics and Astronomy, Monash University, Melbourne, Australia, associated to $^{56}$\\
$^{70}$Pontif{\'\i}cia Universidade Cat{\'o}lica do Rio de Janeiro (PUC-Rio), Rio de Janeiro, Brazil, associated to $^{2}$\\
$^{71}$Physics and Micro Electronic College, Hunan University, Changsha City, China, associated to $^{7}$\\
$^{72}$Guangdong Provincial Key Laboratory of Nuclear Science, Guangdong-Hong Kong Joint Laboratory of Quantum Matter, Institute of Quantum Matter, South China Normal University, Guangzhou, China, associated to $^{3}$\\
$^{73}$School of Physics and Technology, Wuhan University, Wuhan, China, associated to $^{3}$\\
$^{74}$Departamento de Fisica , Universidad Nacional de Colombia, Bogota, Colombia, associated to $^{13}$\\
$^{75}$Universit{\"a}t Bonn - Helmholtz-Institut f{\"u}r Strahlen und Kernphysik, Bonn, Germany, associated to $^{17}$\\
$^{76}$Institut f{\"u}r Physik, Universit{\"a}t Rostock, Rostock, Germany, associated to $^{17}$\\
$^{77}$Eotvos Lorand University, Budapest, Hungary, associated to $^{48}$\\
$^{78}$INFN Sezione di Perugia, Perugia, Italy, associated to $^{21}$\\
$^{79}$Van Swinderen Institute, University of Groningen, Groningen, Netherlands, associated to $^{32}$\\
$^{80}$Universiteit Maastricht, Maastricht, Netherlands, associated to $^{32}$\\
$^{81}$National Research Centre Kurchatov Institute, Moscow, Russia, associated to $^{41}$\\
$^{82}$National Research University Higher School of Economics, Moscow, Russia, associated to $^{42}$\\
$^{83}$National University of Science and Technology ``MISIS'', Moscow, Russia, associated to $^{41}$\\
$^{84}$National Research Tomsk Polytechnic University, Tomsk, Russia, associated to $^{41}$\\
$^{85}$DS4DS, La Salle, Universitat Ramon Llull, Barcelona, Spain, associated to $^{45}$\\
$^{86}$Department of Physics and Astronomy, Uppsala University, Uppsala, Sweden, associated to $^{59}$\\
$^{87}$University of Michigan, Ann Arbor, United States, associated to $^{68}$\\
\bigskip
$^{a}$Universidade Federal do Tri{\^a}ngulo Mineiro (UFTM), Uberaba-MG, Brazil\\
$^{b}$Hangzhou Institute for Advanced Study, UCAS, Hangzhou, China\\
$^{c}$Universit{\`a} di Bari, Bari, Italy\\
$^{d}$Universit{\`a} di Bologna, Bologna, Italy\\
$^{e}$Universit{\`a} di Cagliari, Cagliari, Italy\\
$^{f}$Universit{\`a} di Ferrara, Ferrara, Italy\\
$^{g}$Universit{\`a} di Firenze, Firenze, Italy\\
$^{h}$Universit{\`a} di Genova, Genova, Italy\\
$^{i}$Universit{\`a} degli Studi di Milano, Milano, Italy\\
$^{j}$Universit{\`a} di Milano Bicocca, Milano, Italy\\
$^{k}$Universit{\`a} di Modena e Reggio Emilia, Modena, Italy\\
$^{l}$Universit{\`a} di Padova, Padova, Italy\\
$^{m}$Scuola Normale Superiore, Pisa, Italy\\
$^{n}$Universit{\`a} di Pisa, Pisa, Italy\\
$^{o}$Universit{\`a} della Basilicata, Potenza, Italy\\
$^{p}$Universit{\`a} di Roma Tor Vergata, Roma, Italy\\
$^{q}$Universit{\`a} di Siena, Siena, Italy\\
$^{r}$Universit{\`a} di Urbino, Urbino, Italy\\
$^{s}$MSU - Iligan Institute of Technology (MSU-IIT), Iligan, Philippines\\
$^{t}$P.N. Lebedev Physical Institute, Russian Academy of Science (LPI RAS), Moscow, Russia\\
$^{u}$Novosibirsk State University, Novosibirsk, Russia\\
\medskip
$ ^{\dagger}$Deceased
}
\end{flushleft}

==> LHCb_Authorship_DD-MMM-20YY.tex <==
% ===============================================================================
% Purpose: example of authorlist for LHCb template
% Author:
% Created on: 2009-09-24
% ===============================================================================

%\documentclass[a4paper]{article}
%\setlength{\oddsidemargin}{0cm}
%\setlength{\evensidemargin}{0cm}
%\setlength{\textwidth}{16.5cm}
%\setlength{\parindent}{0cm}
%\begin{document}
\centerline{\large\normalfont\bfseries LHCb collaboration}
\begin{flushleft}
\small
%-- LHCb Authorlist, Example typesetting
%-- 
A.~N.~Other$^{1}$.\bigskip\newline{\it
\footnotesize
$ ^{1}$University of nowhere\\
}
%-- 
%-- 
\end{flushleft}
%\end{document}




==> lhcb-symbols-list.tex <==
% This is an automatically generated appendix to template.tex. 
% When included it will show all the symbols defined in lhcb-symbols-def.tex.
%
% To regenerate with the latest definitions run the script python listsymbols.py

\section{List of all symbols}
\label{sec:listofsymbols}
\subsection{Experiments}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash lhcb} & \lhcb & \texttt{\textbackslash atlas} & \atlas & \texttt{\textbackslash cms} & \cms \\
\texttt{\textbackslash alice} & \alice & \texttt{\textbackslash babar} & \babar & \texttt{\textbackslash belle} & \belle \\
\texttt{\textbackslash belletwo} & \belletwo & \texttt{\textbackslash besiii} & \besiii & \texttt{\textbackslash cleo} & \cleo \\
\texttt{\textbackslash cdf} & \cdf & \texttt{\textbackslash dzero} & \dzero & \texttt{\textbackslash aleph} & \aleph \\
\texttt{\textbackslash delphi} & \delphi & \texttt{\textbackslash opal} & \opal & \texttt{\textbackslash lthree} & \lthree \\
\texttt{\textbackslash sld} & \sld & \texttt{\textbackslash cern} & \cern & \texttt{\textbackslash lhc} & \lhc \\
\texttt{\textbackslash lep} & \lep & \texttt{\textbackslash tevatron} & \tevatron & \texttt{\textbackslash bfactories} & \bfactories \\
\texttt{\textbackslash bfactory} & \bfactory & \texttt{\textbackslash upgradeone} & \upgradeone & \texttt{\textbackslash upgradetwo} & \upgradetwo \\
\end{tabular*}

\subsubsection{LHCb sub-detectors and sub-systems}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash velo} & \velo & \texttt{\textbackslash rich} & \rich & \texttt{\textbackslash richone} & \richone \\
\texttt{\textbackslash richtwo} & \richtwo & \texttt{\textbackslash ttracker} & \ttracker & \texttt{\textbackslash intr} & \intr \\
\texttt{\textbackslash st} & \st & \texttt{\textbackslash ot} & \ot & \texttt{\textbackslash herschel} & \herschel \\
\texttt{\textbackslash spd} & \spd & \texttt{\textbackslash presh} & \presh & \texttt{\textbackslash ecal} & \ecal \\
\texttt{\textbackslash hcal} & \hcal & \texttt{\textbackslash MagUp} & \MagUp & \texttt{\textbackslash MagDown} & \MagDown \\
\texttt{\textbackslash ode} & \ode & \texttt{\textbackslash daq} & \daq & \texttt{\textbackslash tfc} & \tfc \\
\texttt{\textbackslash ecs} & \ecs & \texttt{\textbackslash lone} & \lone & \texttt{\textbackslash hlt} & \hlt \\
\texttt{\textbackslash hltone} & \hltone & \texttt{\textbackslash hlttwo} & \hlttwo &  \\
\end{tabular*}

\subsection{Particles}
\subsubsection{Leptons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash electron} & \electron & \texttt{\textbackslash en} & \en & \texttt{\textbackslash ep} & \ep \\
\texttt{\textbackslash epm} & \epm & \texttt{\textbackslash emp} & \emp & \texttt{\textbackslash epem} & \epem \\
\texttt{\textbackslash muon} & \muon & \texttt{\textbackslash mup} & \mup & \texttt{\textbackslash mun} & \mun \\
\texttt{\textbackslash mupm} & \mupm & \texttt{\textbackslash mump} & \mump & \texttt{\textbackslash mumu} & \mumu \\
\texttt{\textbackslash tauon} & \tauon & \texttt{\textbackslash taup} & \taup & \texttt{\textbackslash taum} & \taum \\
\texttt{\textbackslash taupm} & \taupm & \texttt{\textbackslash taump} & \taump & \texttt{\textbackslash tautau} & \tautau \\
\texttt{\textbackslash lepton} & \lepton & \texttt{\textbackslash ellm} & \ellm & \texttt{\textbackslash ellp} & \ellp \\
\texttt{\textbackslash ellpm} & \ellpm & \texttt{\textbackslash ellmp} & \ellmp & \texttt{\textbackslash ellell} & \ellell \\
\texttt{\textbackslash neu} & \neu & \texttt{\textbackslash neub} & \neub & \texttt{\textbackslash neue} & \neue \\
\texttt{\textbackslash neueb} & \neueb & \texttt{\textbackslash neum} & \neum & \texttt{\textbackslash neumb} & \neumb \\
\texttt{\textbackslash neut} & \neut & \texttt{\textbackslash neutb} & \neutb & \texttt{\textbackslash neul} & \neul \\
\texttt{\textbackslash neulb} & \neulb &  \\
\end{tabular*}

\subsubsection{Gauge bosons and scalars}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash g} & \g & \texttt{\textbackslash H} & \H & \texttt{\textbackslash Hp} & \Hp \\
\texttt{\textbackslash Hm} & \Hm & \texttt{\textbackslash Hpm} & \Hpm & \texttt{\textbackslash W} & \W \\
\texttt{\textbackslash Wp} & \Wp & \texttt{\textbackslash Wm} & \Wm & \texttt{\textbackslash Wpm} & \Wpm \\
\texttt{\textbackslash Z} & \Z &  \\
\end{tabular*}

\subsubsection{Quarks}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash quark} & \quark & \texttt{\textbackslash quarkbar} & \quarkbar & \texttt{\textbackslash qqbar} & \qqbar \\
\texttt{\textbackslash uquark} & \uquark & \texttt{\textbackslash uquarkbar} & \uquarkbar & \texttt{\textbackslash uubar} & \uubar \\
\texttt{\textbackslash dquark} & \dquark & \texttt{\textbackslash dquarkbar} & \dquarkbar & \texttt{\textbackslash ddbar} & \ddbar \\
\texttt{\textbackslash squark} & \squark & \texttt{\textbackslash squarkbar} & \squarkbar & \texttt{\textbackslash ssbar} & \ssbar \\
\texttt{\textbackslash cquark} & \cquark & \texttt{\textbackslash cquarkbar} & \cquarkbar & \texttt{\textbackslash ccbar} & \ccbar \\
\texttt{\textbackslash bquark} & \bquark & \texttt{\textbackslash bquarkbar} & \bquarkbar & \texttt{\textbackslash bbbar} & \bbbar \\
\texttt{\textbackslash tquark} & \tquark & \texttt{\textbackslash tquarkbar} & \tquarkbar & \texttt{\textbackslash ttbar} & \ttbar \\
\end{tabular*}

\subsubsection{Light mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash hadron} & \hadron & \texttt{\textbackslash pion} & \pion & \texttt{\textbackslash piz} & \piz \\
\texttt{\textbackslash pip} & \pip & \texttt{\textbackslash pim} & \pim & \texttt{\textbackslash pipm} & \pipm \\
\texttt{\textbackslash pimp} & \pimp & \texttt{\textbackslash rhomeson} & \rhomeson & \texttt{\textbackslash rhoz} & \rhoz \\
\texttt{\textbackslash rhop} & \rhop & \texttt{\textbackslash rhom} & \rhom & \texttt{\textbackslash rhopm} & \rhopm \\
\texttt{\textbackslash rhomp} & \rhomp & \texttt{\textbackslash kaon} & \kaon & \texttt{\textbackslash Kbar} & \Kbar \\
\texttt{\textbackslash Kb} & \Kb & \texttt{\textbackslash KorKbar} & \KorKbar & \texttt{\textbackslash Kz} & \Kz \\
\texttt{\textbackslash Kzb} & \Kzb & \texttt{\textbackslash Kp} & \Kp & \texttt{\textbackslash Km} & \Km \\
\texttt{\textbackslash Kpm} & \Kpm & \texttt{\textbackslash Kmp} & \Kmp & \texttt{\textbackslash KS} & \KS \\
\texttt{\textbackslash Vzero} & \Vzero & \texttt{\textbackslash KL} & \KL & \texttt{\textbackslash Kstarz} & \Kstarz \\
\texttt{\textbackslash Kstarzb} & \Kstarzb & \texttt{\textbackslash Kstar} & \Kstar & \texttt{\textbackslash Kstarb} & \Kstarb \\
\texttt{\textbackslash Kstarp} & \Kstarp & \texttt{\textbackslash Kstarm} & \Kstarm & \texttt{\textbackslash Kstarpm} & \Kstarpm \\
\texttt{\textbackslash Kstarmp} & \Kstarmp & \texttt{\textbackslash KorKbarz} & \KorKbarz & \texttt{\textbackslash etaz} & \etaz \\
\texttt{\textbackslash etapr} & \etapr & \texttt{\textbackslash phiz} & \phiz & \texttt{\textbackslash omegaz} & \omegaz \\
\end{tabular*}

\subsubsection{Charmed mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Dbar} & \Dbar & \texttt{\textbackslash D} & \D & \texttt{\textbackslash Db} & \Db \\
\texttt{\textbackslash DorDbar} & \DorDbar & \texttt{\textbackslash Dz} & \Dz & \texttt{\textbackslash Dzb} & \Dzb \\
\texttt{\textbackslash Dp} & \Dp & \texttt{\textbackslash Dm} & \Dm & \texttt{\textbackslash Dpm} & \Dpm \\
\texttt{\textbackslash Dmp} & \Dmp & \texttt{\textbackslash DpDm} & \DpDm & \texttt{\textbackslash Dstar} & \Dstar \\
\texttt{\textbackslash Dstarb} & \Dstarb & \texttt{\textbackslash Dstarz} & \Dstarz & \texttt{\textbackslash Dstarzb} & \Dstarzb \\
\texttt{\textbackslash theDstarz} & \theDstarz & \texttt{\textbackslash theDstarzb} & \theDstarzb & \texttt{\textbackslash Dstarp} & \Dstarp \\
\texttt{\textbackslash Dstarm} & \Dstarm & \texttt{\textbackslash Dstarpm} & \Dstarpm & \texttt{\textbackslash Dstarmp} & \Dstarmp \\
\texttt{\textbackslash theDstarp} & \theDstarp & \texttt{\textbackslash theDstarm} & \theDstarm & \texttt{\textbackslash theDstarpm} & \theDstarpm \\
\texttt{\textbackslash theDstarmp} & \theDstarmp & \texttt{\textbackslash Ds} & \Ds & \texttt{\textbackslash Dsp} & \Dsp \\
\texttt{\textbackslash Dsm} & \Dsm & \texttt{\textbackslash Dspm} & \Dspm & \texttt{\textbackslash Dsmp} & \Dsmp \\
\texttt{\textbackslash Dss} & \Dss & \texttt{\textbackslash Dssp} & \Dssp & \texttt{\textbackslash Dssm} & \Dssm \\
\texttt{\textbackslash Dsspm} & \Dsspm & \texttt{\textbackslash Dssmp} & \Dssmp & \texttt{\textbackslash DporDsp} & \DporDsp \\
\texttt{\textbackslash DmorDsm} & \DmorDsm & \texttt{\textbackslash DpmorDspm} & \DpmorDspm &  \\
\end{tabular*}

\subsubsection{Beauty mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash B} & \B & \texttt{\textbackslash Bbar} & \Bbar & \texttt{\textbackslash Bb} & \Bb \\
\texttt{\textbackslash BorBbar} & \BorBbar & \texttt{\textbackslash Bz} & \Bz & \texttt{\textbackslash Bzb} & \Bzb \\
\texttt{\textbackslash Bd} & \Bd & \texttt{\textbackslash Bdb} & \Bdb & \texttt{\textbackslash BdorBdbar} & \BdorBdbar \\
\texttt{\textbackslash Bu} & \Bu & \texttt{\textbackslash Bub} & \Bub & \texttt{\textbackslash Bp} & \Bp \\
\texttt{\textbackslash Bm} & \Bm & \texttt{\textbackslash Bpm} & \Bpm & \texttt{\textbackslash Bmp} & \Bmp \\
\texttt{\textbackslash Bs} & \Bs & \texttt{\textbackslash Bsb} & \Bsb & \texttt{\textbackslash BsorBsbar} & \BsorBsbar \\
\texttt{\textbackslash Bc} & \Bc & \texttt{\textbackslash Bcp} & \Bcp & \texttt{\textbackslash Bcm} & \Bcm \\
\texttt{\textbackslash Bcpm} & \Bcpm & \texttt{\textbackslash Bds} & \Bds & \texttt{\textbackslash Bdsb} & \Bdsb \\
\texttt{\textbackslash BdorBs} & \BdorBs & \texttt{\textbackslash BdorBsbar} & \BdorBsbar &  \\
\end{tabular*}

\subsubsection{Onia}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash jpsi} & \jpsi & \texttt{\textbackslash psitwos} & \psitwos & \texttt{\textbackslash psiprpr} & \psiprpr \\
\texttt{\textbackslash etac} & \etac & \texttt{\textbackslash psires} & \psires & \texttt{\textbackslash chic} & \chic \\
\texttt{\textbackslash chiczero} & \chiczero & \texttt{\textbackslash chicone} & \chicone & \texttt{\textbackslash chictwo} & \chictwo \\
\texttt{\textbackslash chicJ} & \chicJ & \texttt{\textbackslash Upsilonres} & \Upsilonres & \texttt{\textbackslash OneS} & \OneS \\
\texttt{\textbackslash TwoS} & \TwoS & \texttt{\textbackslash ThreeS} & \ThreeS & \texttt{\textbackslash FourS} & \FourS \\
\texttt{\textbackslash FiveS} & \FiveS & \texttt{\textbackslash chib} & \chib & \texttt{\textbackslash chibzero} & \chibzero \\
\texttt{\textbackslash chibone} & \chibone & \texttt{\textbackslash chibtwo} & \chibtwo & \texttt{\textbackslash chibJ} & \chibJ \\
\texttt{\textbackslash theX} & \theX &  \\
\end{tabular*}

\subsubsection{Light Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash proton} & \proton & \texttt{\textbackslash antiproton} & \antiproton & \texttt{\textbackslash neutron} & \neutron \\
\texttt{\textbackslash antineutron} & \antineutron & \texttt{\textbackslash Deltares} & \Deltares & \texttt{\textbackslash Deltaresbar} & \Deltaresbar \\
\texttt{\textbackslash Lz} & \Lz & \texttt{\textbackslash Lbar} & \Lbar & \texttt{\textbackslash LorLbar} & \LorLbar \\
\texttt{\textbackslash Lambdares} & \Lambdares & \texttt{\textbackslash Lambdaresbar} & \Lambdaresbar & \texttt{\textbackslash Sigmares} & \Sigmares \\
\texttt{\textbackslash Sigmaz} & \Sigmaz & \texttt{\textbackslash Sigmap} & \Sigmap & \texttt{\textbackslash Sigmam} & \Sigmam \\
\texttt{\textbackslash Sigmaresbar} & \Sigmaresbar & \texttt{\textbackslash Sigmabarz} & \Sigmabarz & \texttt{\textbackslash Sigmabarp} & \Sigmabarp \\
\texttt{\textbackslash Sigmabarm} & \Sigmabarm & \texttt{\textbackslash Xires} & \Xires & \texttt{\textbackslash Xiz} & \Xiz \\
\texttt{\textbackslash Xim} & \Xim & \texttt{\textbackslash Xiresbar} & \Xiresbar & \texttt{\textbackslash Xibarz} & \Xibarz \\
\texttt{\textbackslash Xibarp} & \Xibarp & \texttt{\textbackslash Omegares} & \Omegares & \texttt{\textbackslash Omegaresbar} & \Omegaresbar \\
\texttt{\textbackslash Omegam} & \Omegam & \texttt{\textbackslash Omegabarp} & \Omegabarp &  \\
\end{tabular*}

\subsubsection{Charmed Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Lc} & \Lc & \texttt{\textbackslash Lcbar} & \Lcbar & \texttt{\textbackslash Xic} & \Xic \\
\texttt{\textbackslash Xicz} & \Xicz & \texttt{\textbackslash Xicp} & \Xicp & \texttt{\textbackslash Xicbar} & \Xicbar \\
\texttt{\textbackslash Xicbarz} & \Xicbarz & \texttt{\textbackslash Xicbarm} & \Xicbarm & \texttt{\textbackslash Omegac} & \Omegac \\
\texttt{\textbackslash Omegacbar} & \Omegacbar & \texttt{\textbackslash Xicc} & \Xicc & \texttt{\textbackslash Xiccbar} & \Xiccbar \\
\texttt{\textbackslash Xiccp} & \Xiccp & \texttt{\textbackslash Xiccpp} & \Xiccpp & \texttt{\textbackslash Xiccbarm} & \Xiccbarm \\
\texttt{\textbackslash Xiccbarmm} & \Xiccbarmm & \texttt{\textbackslash Omegacc} & \Omegacc & \texttt{\textbackslash Omegaccbar} & \Omegaccbar \\
\texttt{\textbackslash Omegaccc} & \Omegaccc & \texttt{\textbackslash Omegacccbar} & \Omegacccbar &  \\
\end{tabular*}

\subsubsection{Beauty Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Lb} & \Lb & \texttt{\textbackslash Lbbar} & \Lbbar & \texttt{\textbackslash Sigmab} & \Sigmab \\
\texttt{\textbackslash Sigmabp} & \Sigmabp & \texttt{\textbackslash Sigmabz} & \Sigmabz & \texttt{\textbackslash Sigmabm} & \Sigmabm \\
\texttt{\textbackslash Sigmabpm} & \Sigmabpm & \texttt{\textbackslash Sigmabbar} & \Sigmabbar & \texttt{\textbackslash Sigmabbarp} & \Sigmabbarp \\
\texttt{\textbackslash Sigmabbarz} & \Sigmabbarz & \texttt{\textbackslash Sigmabbarm} & \Sigmabbarm & \texttt{\textbackslash Sigmabbarpm} & \Sigmabbarpm \\
\texttt{\textbackslash Xib} & \Xib & \texttt{\textbackslash Xibz} & \Xibz & \texttt{\textbackslash Xibm} & \Xibm \\
\texttt{\textbackslash Xibbar} & \Xibbar & \texttt{\textbackslash Xibbarz} & \Xibbarz & \texttt{\textbackslash Xibbarp} & \Xibbarp \\
\texttt{\textbackslash Omegab} & \Omegab & \texttt{\textbackslash Omegabbar} & \Omegabbar &  \\
\end{tabular*}

\subsection{Physics symbols}
\subsubsection{Decays}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BF} & \BF & \texttt{\textbackslash BR} & \BR & \texttt{\textbackslash BRvis} & \BRvis \\
\texttt{\textbackslash ra} & \ra & \texttt{\textbackslash to} & \to &  \\
\end{tabular*}

\subsubsection{Lifetimes}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tauBs} & \tauBs & \texttt{\textbackslash tauBd} & \tauBd & \texttt{\textbackslash tauBz} & \tauBz \\
\texttt{\textbackslash tauBu} & \tauBu & \texttt{\textbackslash tauDp} & \tauDp & \texttt{\textbackslash tauDz} & \tauDz \\
\texttt{\textbackslash tauL} & \tauL & \texttt{\textbackslash tauH} & \tauH &  \\
\end{tabular*}

\subsubsection{Masses}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash mBd} & \mBd & \texttt{\textbackslash mBp} & \mBp & \texttt{\textbackslash mBs} & \mBs \\
\texttt{\textbackslash mBc} & \mBc & \texttt{\textbackslash mLb} & \mLb &  \\
\end{tabular*}

\subsubsection{EW theory, groups}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash grpsuthree} & \grpsuthree & \texttt{\textbackslash grpsutw} & \grpsutw & \texttt{\textbackslash grpuone} & \grpuone \\
\texttt{\textbackslash ssqtw} & \ssqtw & \texttt{\textbackslash csqtw} & \csqtw & \texttt{\textbackslash stw} & \stw \\
\texttt{\textbackslash ctw} & \ctw & \texttt{\textbackslash ssqtwef} & \ssqtwef & \texttt{\textbackslash csqtwef} & \csqtwef \\
\texttt{\textbackslash stwef} & \stwef & \texttt{\textbackslash ctwef} & \ctwef & \texttt{\textbackslash gv} & \gv \\
\texttt{\textbackslash ga} & \ga & \texttt{\textbackslash order} & \order & \texttt{\textbackslash ordalph} & \ordalph \\
\texttt{\textbackslash ordalsq} & \ordalsq & \texttt{\textbackslash ordalcb} & \ordalcb &  \\
\end{tabular*}

\subsubsection{QCD parameters}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash as} & \as & \texttt{\textbackslash MSb} & \MSb & \texttt{\textbackslash lqcd} & \lqcd \\
\texttt{\textbackslash qsq} & \qsq &  \\
\end{tabular*}

\subsubsection{CKM, \boldmath \CP violation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash eps} & \eps & \texttt{\textbackslash epsK} & \epsK & \texttt{\textbackslash epsB} & \epsB \\
\texttt{\textbackslash epsp} & \epsp & \texttt{\textbackslash CP} & \CP & \texttt{\textbackslash CPT} & \CPT \\
\texttt{\textbackslash T} & \T & \texttt{\textbackslash rhobar} & \rhobar & \texttt{\textbackslash etabar} & \etabar \\
\texttt{\textbackslash Vud} & \Vud & \texttt{\textbackslash Vcd} & \Vcd & \texttt{\textbackslash Vtd} & \Vtd \\
\texttt{\textbackslash Vus} & \Vus & \texttt{\textbackslash Vcs} & \Vcs & \texttt{\textbackslash Vts} & \Vts \\
\texttt{\textbackslash Vub} & \Vub & \texttt{\textbackslash Vcb} & \Vcb & \texttt{\textbackslash Vtb} & \Vtb \\
\texttt{\textbackslash Vuds} & \Vuds & \texttt{\textbackslash Vcds} & \Vcds & \texttt{\textbackslash Vtds} & \Vtds \\
\texttt{\textbackslash Vuss} & \Vuss & \texttt{\textbackslash Vcss} & \Vcss & \texttt{\textbackslash Vtss} & \Vtss \\
\texttt{\textbackslash Vubs} & \Vubs & \texttt{\textbackslash Vcbs} & \Vcbs & \texttt{\textbackslash Vtbs} & \Vtbs \\
\end{tabular*}

\subsubsection{Oscillations}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash dm} & \dm & \texttt{\textbackslash dms} & \dms & \texttt{\textbackslash dmd} & \dmd \\
\texttt{\textbackslash DG} & \DG & \texttt{\textbackslash DGs} & \DGs & \texttt{\textbackslash DGd} & \DGd \\
\texttt{\textbackslash Gs} & \Gs & \texttt{\textbackslash Gd} & \Gd & \texttt{\textbackslash MBq} & \MBq \\
\texttt{\textbackslash DGq} & \DGq & \texttt{\textbackslash Gq} & \Gq & \texttt{\textbackslash dmq} & \dmq \\
\texttt{\textbackslash GL} & \GL & \texttt{\textbackslash GH} & \GH & \texttt{\textbackslash DGsGs} & \DGsGs \\
\texttt{\textbackslash Delm} & \Delm & \texttt{\textbackslash ACP} & \ACP & \texttt{\textbackslash Adir} & \Adir \\
\texttt{\textbackslash Amix} & \Amix & \texttt{\textbackslash ADelta} & \ADelta & \texttt{\textbackslash phid} & \phid \\
\texttt{\textbackslash sinphid} & \sinphid & \texttt{\textbackslash phis} & \phis & \texttt{\textbackslash betas} & \betas \\
\texttt{\textbackslash sbetas} & \sbetas & \texttt{\textbackslash stbetas} & \stbetas & \texttt{\textbackslash stphis} & \stphis \\
\texttt{\textbackslash sinphis} & \sinphis &  \\
\end{tabular*}

\subsubsection{Tagging}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash edet} & \edet & \texttt{\textbackslash erec} & \erec & \texttt{\textbackslash esel} & \esel \\
\texttt{\textbackslash etrg} & \etrg & \texttt{\textbackslash etot} & \etot & \texttt{\textbackslash mistag} & \mistag \\
\texttt{\textbackslash wcomb} & \wcomb & \texttt{\textbackslash etag} & \etag & \texttt{\textbackslash etagcomb} & \etagcomb \\
\texttt{\textbackslash effeff} & \effeff & \texttt{\textbackslash effeffcomb} & \effeffcomb & \texttt{\textbackslash efftag} & \efftag \\
\texttt{\textbackslash effD} & \effD & \texttt{\textbackslash etagprompt} & \etagprompt & \texttt{\textbackslash etagLL} & \etagLL \\
\end{tabular*}

\subsubsection{Key decay channels}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BdToKstmm} & \BdToKstmm & \texttt{\textbackslash BdbToKstmm} & \BdbToKstmm & \texttt{\textbackslash BsToJPsiPhi} & \BsToJPsiPhi \\
\texttt{\textbackslash BdToJPsiKst} & \BdToJPsiKst & \texttt{\textbackslash BdbToJPsiKst} & \BdbToJPsiKst & \texttt{\textbackslash BsPhiGam} & \BsPhiGam \\
\texttt{\textbackslash BdKstGam} & \BdKstGam & \texttt{\textbackslash BTohh} & \BTohh & \texttt{\textbackslash BdTopipi} & \BdTopipi \\
\texttt{\textbackslash BdToKpi} & \BdToKpi & \texttt{\textbackslash BsToKK} & \BsToKK & \texttt{\textbackslash BsTopiK} & \BsTopiK \\
\texttt{\textbackslash Cpipi} & \Cpipi & \texttt{\textbackslash Spipi} & \Spipi & \texttt{\textbackslash CKK} & \CKK \\
\texttt{\textbackslash SKK} & \SKK & \texttt{\textbackslash ADGKK} & \ADGKK &  \\
\end{tabular*}

\subsubsection{Rare decays}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BdKstee} & \BdKstee & \texttt{\textbackslash BdbKstee} & \BdbKstee & \texttt{\textbackslash bsll} & \bsll \\
\texttt{\textbackslash AFB} & \AFB & \texttt{\textbackslash FL} & \FL & \texttt{\textbackslash AT\#1 \textbackslash AT2} & \AT2 \\
\texttt{\textbackslash btosgam} & \btosgam & \texttt{\textbackslash btodgam} & \btodgam & \texttt{\textbackslash Bsmm} & \Bsmm \\
\texttt{\textbackslash Bdmm} & \Bdmm & \texttt{\textbackslash Bsee} & \Bsee & \texttt{\textbackslash Bdee} & \Bdee \\
\texttt{\textbackslash ctl} & \ctl & \texttt{\textbackslash ctk} & \ctk &  \\
\end{tabular*}

\subsubsection{Wilson coefficients and operators}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash C\#1 \textbackslash C9} & \C9 & \texttt{\textbackslash Cp\#1 \textbackslash Cp7} & \Cp7 & \texttt{\textbackslash Ceff\#1 \textbackslash Ceff9  } & \Ceff9   \\
\texttt{\textbackslash Cpeff\#1 \textbackslash Cpeff7} & \Cpeff7 & \texttt{\textbackslash Ope\#1 \textbackslash Ope2} & \Ope2 & \texttt{\textbackslash Opep\#1 \textbackslash Opep7} & \Opep7 \\
\end{tabular*}

\subsubsection{Charm}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash xprime} & \xprime & \texttt{\textbackslash yprime} & \yprime & \texttt{\textbackslash ycp} & \ycp \\
\texttt{\textbackslash agamma} & \agamma & \texttt{\textbackslash dkpicf} & \dkpicf &  \\
\end{tabular*}

\subsubsection{QM}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash bra[1] \textbackslash bra\{a\}} & \bra{a} & \texttt{\textbackslash ket[1] \textbackslash ket\{b\}} & \ket{b} & \texttt{\textbackslash braket[2] \textbackslash braket\{a\}\{b\}} & \braket{a}{b} \\
\end{tabular*}

\subsection{Units (these macros add a small space in front)}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash unit[1] \textbackslash unit\{kg\}   } & \unit{kg}    &  \\
\end{tabular*}

\subsubsection{Energy and momentum }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tev} & \tev & \texttt{\textbackslash gev} & \gev & \texttt{\textbackslash mev} & \mev \\
\texttt{\textbackslash kev} & \kev & \texttt{\textbackslash ev} & \ev & \texttt{\textbackslash gevgev} & \gevgev \\
\texttt{\textbackslash mevc} & \mevc & \texttt{\textbackslash gevc} & \gevc & \texttt{\textbackslash mevcc} & \mevcc \\
\texttt{\textbackslash gevcc} & \gevcc & \texttt{\textbackslash gevgevcc} & \gevgevcc & \texttt{\textbackslash gevgevcccc} & \gevgevcccc \\
\end{tabular*}

\subsubsection{Distance and area (these macros add a small space)}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash km} & \km & \texttt{\textbackslash m} & \m & \texttt{\textbackslash ma} & \ma \\
\texttt{\textbackslash cm} & \cm & \texttt{\textbackslash cma} & \cma & \texttt{\textbackslash mm} & \mm \\
\texttt{\textbackslash mma} & \mma & \texttt{\textbackslash mum} & \mum & \texttt{\textbackslash muma} & \muma \\
\texttt{\textbackslash nm} & \nm & \texttt{\textbackslash fm} & \fm & \texttt{\textbackslash barn} & \barn \\
\texttt{\textbackslash mbarn} & \mbarn & \texttt{\textbackslash mub} & \mub & \texttt{\textbackslash nb} & \nb \\
\texttt{\textbackslash invnb} & \invnb & \texttt{\textbackslash pb} & \pb & \texttt{\textbackslash invpb} & \invpb \\
\texttt{\textbackslash fb} & \fb & \texttt{\textbackslash invfb} & \invfb & \texttt{\textbackslash ab} & \ab \\
\texttt{\textbackslash invab} & \invab &  \\
\end{tabular*}

\subsubsection{Time }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash sec} & \sec & \texttt{\textbackslash ms} & \ms & \texttt{\textbackslash mus} & \mus \\
\texttt{\textbackslash ns} & \ns & \texttt{\textbackslash ps} & \ps & \texttt{\textbackslash fs} & \fs \\
\texttt{\textbackslash mhz} & \mhz & \texttt{\textbackslash khz} & \khz & \texttt{\textbackslash hz} & \hz \\
\texttt{\textbackslash invps} & \invps & \texttt{\textbackslash invns} & \invns & \texttt{\textbackslash yr} & \yr \\
\texttt{\textbackslash hr} & \hr &  \\
\end{tabular*}

\subsubsection{Temperature}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash degc} & \degc & \texttt{\textbackslash degk} & \degk &  \\
\end{tabular*}

\subsubsection{Material lengths, radiation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Xrad} & \Xrad & \texttt{\textbackslash NIL} & \NIL & \texttt{\textbackslash mip} & \mip \\
\texttt{\textbackslash neutroneq} & \neutroneq & \texttt{\textbackslash neqcmcm} & \neqcmcm & \texttt{\textbackslash kRad} & \kRad \\
\texttt{\textbackslash MRad} & \MRad & \texttt{\textbackslash ci} & \ci & \texttt{\textbackslash mci} & \mci \\
\end{tabular*}

\subsubsection{Uncertainties}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash sx} & \sx & \texttt{\textbackslash sy} & \sy & \texttt{\textbackslash sz} & \sz \\
\texttt{\textbackslash stat} & \stat & \texttt{\textbackslash syst} & \syst & \texttt{\textbackslash lumi} & \lumi \\
\end{tabular*}

\subsubsection{Maths}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash order} & \order & \texttt{\textbackslash chisq} & \chisq & \texttt{\textbackslash chisqndf} & \chisqndf \\
\texttt{\textbackslash chisqip} & \chisqip & \texttt{\textbackslash chisqvs} & \chisqvs & \texttt{\textbackslash chisqvtx} & \chisqvtx \\
\texttt{\textbackslash chisqvtxndf} & \chisqvtxndf & \texttt{\textbackslash deriv} & \deriv & \texttt{\textbackslash gsim} & \gsim \\
\texttt{\textbackslash lsim} & \lsim & \texttt{\textbackslash mean[1] \textbackslash mean\{x\}} & \mean{x} & \texttt{\textbackslash abs[1] \textbackslash abs\{x\}} & \abs{x} \\
\texttt{\textbackslash Real} & \Real & \texttt{\textbackslash Imag} & \Imag & \texttt{\textbackslash PDF} & \PDF \\
\texttt{\textbackslash sPlot} & \sPlot & \texttt{\textbackslash sFit} & \sFit &  \\
\end{tabular*}

\subsection{Kinematics}
\subsubsection{Energy, Momenta}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Ebeam} & \Ebeam & \texttt{\textbackslash sqs} & \sqs & \texttt{\textbackslash sqsnn} & \sqsnn \\
\texttt{\textbackslash pt} & \pt & \texttt{\textbackslash ptsq} & \ptsq & \texttt{\textbackslash ptot} & \ptot \\
\texttt{\textbackslash et} & \et & \texttt{\textbackslash mt} & \mt & \texttt{\textbackslash dpp} & \dpp \\
\texttt{\textbackslash msq} & \msq & \texttt{\textbackslash dedx} & \dedx &  \\
\end{tabular*}

\subsubsection{PID}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash dllkpi} & \dllkpi & \texttt{\textbackslash dllppi} & \dllppi & \texttt{\textbackslash dllepi} & \dllepi \\
\texttt{\textbackslash dllmupi} & \dllmupi &  \\
\end{tabular*}

\subsubsection{Geometry}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash degrees} & \degrees & \texttt{\textbackslash murad} & \murad & \texttt{\textbackslash mrad} & \mrad \\
\texttt{\textbackslash rad} & \rad &  \\
\end{tabular*}

\subsubsection{Accelerator}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash betastar} & \betastar & \texttt{\textbackslash lum} & \lum & \texttt{\textbackslash intlum[1] \textbackslash intlum\{2 \,\invfb\}} & \intlum{2 \,\invfb} \\
\end{tabular*}

\subsection{Software}
\subsubsection{Programs}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash bcvegpy} & \bcvegpy & \texttt{\textbackslash boole} & \boole & \texttt{\textbackslash brunel} & \brunel \\
\texttt{\textbackslash davinci} & \davinci & \texttt{\textbackslash dirac} & \dirac & \texttt{\textbackslash evtgen} & \evtgen \\
\texttt{\textbackslash fewz} & \fewz & \texttt{\textbackslash fluka} & \fluka & \texttt{\textbackslash ganga} & \ganga \\
\texttt{\textbackslash gaudi} & \gaudi & \texttt{\textbackslash gauss} & \gauss & \texttt{\textbackslash geant} & \geant \\
\texttt{\textbackslash hepmc} & \hepmc & \texttt{\textbackslash herwig} & \herwig & \texttt{\textbackslash moore} & \moore \\
\texttt{\textbackslash neurobayes} & \neurobayes & \texttt{\textbackslash photos} & \photos & \texttt{\textbackslash powheg} & \powheg \\
\texttt{\textbackslash pythia} & \pythia & \texttt{\textbackslash resbos} & \resbos & \texttt{\textbackslash roofit} & \roofit \\
\texttt{\textbackslash root} & \root & \texttt{\textbackslash spice} & \spice & \texttt{\textbackslash urania} & \urania \\
\end{tabular*}

\subsubsection{Languages}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash cpp} & \cpp & \texttt{\textbackslash ruby} & \ruby & \texttt{\textbackslash fortran} & \fortran \\
\texttt{\textbackslash svn} & \svn & \texttt{\textbackslash git} & \git & \texttt{\textbackslash latex} & \latex \\
\end{tabular*}

\subsubsection{Data processing}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash kbit} & \kbit & \texttt{\textbackslash kbps} & \kbps & \texttt{\textbackslash kbytes} & \kbytes \\
\texttt{\textbackslash kbyps} & \kbyps & \texttt{\textbackslash mbit} & \mbit & \texttt{\textbackslash mbps} & \mbps \\
\texttt{\textbackslash mbytes} & \mbytes & \texttt{\textbackslash mbyps} & \mbyps & \texttt{\textbackslash gbit} & \gbit \\
\texttt{\textbackslash gbps} & \gbps & \texttt{\textbackslash gbytes} & \gbytes & \texttt{\textbackslash gbyps} & \gbyps \\
\texttt{\textbackslash tbit} & \tbit & \texttt{\textbackslash tbps} & \tbps & \texttt{\textbackslash tbytes} & \tbytes \\
\texttt{\textbackslash tbyps} & \tbyps & \texttt{\textbackslash dst} & \dst &  \\
\end{tabular*}

\subsection{Detector related}
\subsubsection{Detector technologies}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash nonn} & \nonn & \texttt{\textbackslash ponn} & \ponn & \texttt{\textbackslash nonp} & \nonp \\
\texttt{\textbackslash cvd} & \cvd & \texttt{\textbackslash mwpc} & \mwpc & \texttt{\textbackslash gem} & \gem \\
\end{tabular*}

\subsubsection{Detector components, electronics}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tell1} & \tell1 & \texttt{\textbackslash ukl1} & \ukl1 & \texttt{\textbackslash beetle} & \beetle \\
\texttt{\textbackslash otis} & \otis & \texttt{\textbackslash croc} & \croc & \texttt{\textbackslash carioca} & \carioca \\
\texttt{\textbackslash dialog} & \dialog & \texttt{\textbackslash sync} & \sync & \texttt{\textbackslash cardiac} & \cardiac \\
\texttt{\textbackslash gol} & \gol & \texttt{\textbackslash vcsel} & \vcsel & \texttt{\textbackslash ttc} & \ttc \\
\texttt{\textbackslash ttcrx} & \ttcrx & \texttt{\textbackslash hpd} & \hpd & \texttt{\textbackslash pmt} & \pmt \\
\texttt{\textbackslash specs} & \specs & \texttt{\textbackslash elmb} & \elmb & \texttt{\textbackslash fpga} & \fpga \\
\texttt{\textbackslash plc} & \plc & \texttt{\textbackslash rasnik} & \rasnik & \texttt{\textbackslash elmb} & \elmb \\
\texttt{\textbackslash can} & \can & \texttt{\textbackslash lvds} & \lvds & \texttt{\textbackslash ntc} & \ntc \\
\texttt{\textbackslash adc} & \adc & \texttt{\textbackslash led} & \led & \texttt{\textbackslash ccd} & \ccd \\
\texttt{\textbackslash hv} & \hv & \texttt{\textbackslash lv} & \lv & \texttt{\textbackslash pvss} & \pvss \\
\texttt{\textbackslash cmos} & \cmos & \texttt{\textbackslash fifo} & \fifo & \texttt{\textbackslash ccpc} & \ccpc \\
\end{tabular*}

\subsubsection{Chemical symbols}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash cfourften} & \cfourften & \texttt{\textbackslash cffour} & \cffour & \texttt{\textbackslash cotwo} & \cotwo \\
\texttt{\textbackslash csixffouteen} & \csixffouteen & \texttt{\textbackslash mgftwo} & \mgftwo & \texttt{\textbackslash siotwo} & \siotwo \\
\end{tabular*}

\subsection{Special Text }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash eg} & \eg & \texttt{\textbackslash ie} & \ie & \texttt{\textbackslash etal} & \etal \\
\texttt{\textbackslash etc} & \etc & \texttt{\textbackslash cf} & \cf & \texttt{\textbackslash ffp} & \ffp \\
\texttt{\textbackslash vs} & \vs &  \\
\end{tabular*}

\subsubsection{Helpful to align numbers in tables}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash phz} & \phz &  \\
\end{tabular*}



==> refs_main.tex <==

\ifx\mcitethebibliography\mciteundefinedmacro
\PackageError{LHCb.bst}{mciteplus.sty has not been loaded}
{This bibstyle requires the use of the mciteplus package.}\fi
\providecommand{\href}[2]{#2}
\begin{mcitethebibliography}{100}
\mciteSetBstSublistMode{n}
\mciteSetBstMaxWidthForm{subitem}{\alph{mcitesubitemcount})}
\mciteSetBstSublistLabelBeginEnd{\mcitemaxwidthsubitemform\space}
{\relax}{\relax}


\bibitem{GellMann:1964nj}
M.~Gell-Mann, \ifthenelse{\boolean{articletitles}}{\emph{{A~schematic model of
  baryons and mesons}},
  }{}\href{https://doi.org/10.1016/S0031-9163(64)92001-3}{Phys.\ Lett.\
  \textbf{8} 214--215} (1964)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Zweig:352337}
G.~Zweig, \ifthenelse{\boolean{articletitles}}{\emph{{An SU$_3$ model for
  strong interaction symmetry and its breaking; Version 1,}}, }{} Tech. Rep.
  \href{http://cds.cern.ch/record/352337}{CERN-TH-401}, CERN, Geneva,
  1964\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Zweig:570209}
G.~Zweig, \ifthenelse{\boolean{articletitles}}{\emph{{An SU$_3$ model for
  strong interaction symmetry and its breaking; Version 2,}}, }{} Tech. Rep.
  \href{http://cds.cern.ch/record/570209}{CERN-TH-412}, CERN, Geneva,
  1964\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Jaffe:1976ig}
R.~L. Jaffe, \ifthenelse{\boolean{articletitles}}{\emph{{Multiquark hadrons. I.
  Phenomenology of $\PQ^2\bar{\PQ}^2$~mesons}},
  }{}\href{https://doi.org/10.1103/PhysRevD.15.267}{Phys.\ Rev.\  \textbf{D15}
  267--280} (1977)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Jaffe:1976ih}
R.~L. Jaffe, \ifthenelse{\boolean{articletitles}}{\emph{{Multi-quark hadrons.
  2.~Methods}}, }{}\href{https://doi.org/10.1103/PhysRevD.15.281}{Phys.\ Rev.\
  \textbf{D15} 281--289} (1977)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Rossi:1977cy}
G.~C. Rossi and G.~Veneziano,
  \ifthenelse{\boolean{articletitles}}{\emph{{A~possible description of baryon
  dynamics in dual and gauge theories}},
  }{}\href{https://doi.org/10.1016/0550-3213(77)90178-X}{Nucl.\ Phys.\
  \textbf{B123} 507--545} (1977)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Jaffe:1977cv}
R.~L. Jaffe, \ifthenelse{\boolean{articletitles}}{\emph{{
  $\PQ^2\bar{\PQ}^2$~resonances in the~baryon\nobreakdash-antibaryon system}},
  }{}\href{https://doi.org/10.1103/PhysRevD.17.1444}{Phys.\ Rev.\  \textbf{D17}
  1444--1458} (1978)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Lipkin:1987sk}
H.~J. Lipkin, \ifthenelse{\boolean{articletitles}}{\emph{{New~possibilities for
  exotic hadrons - anticharmed strange baryons}},
  }{}\href{https://doi.org/10.1016/0370-2693(87)90055-4}{Phys.\ Lett.\
  \textbf{B195} 484--488} (1987)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Choi:2003ue}
Belle collaboration, S.~K. Choi {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of a~narrow
  charmoniumlike state in exclusive
  \mbox{$\decay{\B^{\pm}}{\kaon^{\pm}\pip\pim\jpsi}$}~decays}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.91.262001}{Phys.\ Rev.\ Lett.\
  \textbf{91} 262001} (2003)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Choi:2007wga}
Belle collaboration, S.~K. Choi {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of a~resonancelike
  structure in the~\mbox{$\Ppi^\pm\Ppsi^\prime$}~mass distribution in exclusive
  \mbox{$\decay{\B}{\kaon\Ppi^{\pm}\Ppsi^{\prime}}$}~decays}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.100.142001}{Phys.\ Rev.\ Lett.\
  \textbf{100} 142001} (2008)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Belle:2008qeq}
Belle collaboration, R.~Mizuk {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of two
  resonance\nobreakdash-like structures in the~\mbox{$\pip\chicone$}~mass
  distribution in exclusive \mbox{$\decay{\Bdb}{\Km\pip\chicone}$}~decays}},
  }{}\href{https://doi.org/10.1103/PhysRevD.78.072004}{Phys.\ Rev.\
  \textbf{D78} 072004} (2008)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Aaltonen:2009tz}
CDF collaboration, T.~Aaltonen {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Evidence for a~narrow
  near\nobreakdash-threshold structure in the~$\jpsi\Pphi$~mass spectrum in
  \mbox{$\decay{\Bu}{\jpsi\Pphi\Kp}$}~decays}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.102.242002}{Phys.\ Rev.\ Lett.\
  \textbf{102} 242002} (2009)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Belle:2011aa}
Belle collaboration, A.~Bondar {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of two charged
  bottomonium\nobreakdash-like resonances in $\PUpsilon(5\PS)$~decays}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.108.122001}{Phys.\ Rev.\ Lett.\
  \textbf{108} 122001} (2012)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Ablikim:2013mio}
BESIII collaboration, M.~Ablikim {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of a~charged
  charmoniumlike structure in \mbox{$\decay{\epem}{\pip\pim\jpsi}$} at
  \mbox{$\sqs=4.26\gev$} }},
  }{}\href{https://doi.org/10.1103/PhysRevLett.110.252001}{Phys.\ Rev.\ Lett.\
  \textbf{110} 252001} (2013)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{BESIII:2013ouc}
BESIII collaboration, M.~Ablikim {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of a~charged
  charmoniumlike structure \mbox{$\Z_{\cquark}(4020)$} and search for
  the~\mbox{$Z_{\cquark}(3900)$} in
  \mbox{$\decay{\epem}{\pip\pim\Ph_{\cquark}}$} }},
  }{}\href{https://doi.org/10.1103/PhysRevLett.111.242001}{Phys.\ Rev.\ Lett.\
  \textbf{111} 242001} (2013)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{BESIII:2013mhi}
BESIII collaboration, M.~Ablikim {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of a~charged
  charmoniumlike structure in
  \mbox{$\decay{\epem}{\left(\Dstar\Dstarb\right)^{\pm}\pion^{\mp}}$}
  at~\mbox{$\sqs=4.26\gev$} }},
  }{}\href{https://doi.org/10.1103/PhysRevLett.112.132001}{Phys.\ Rev.\ Lett.\
  \textbf{112} 132001} (2014)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Abazov:2013xda}
D0 collaboration, V.~M. Abazov {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Search for the~$\PX(4140)$~state
  in \mbox{$\decay{\Bu}{\jpsi\Pphi\Kp}$}~decays with the D0 Detector}},
  }{}\href{https://doi.org/10.1103/PhysRevD.89.012004}{Phys.\ Rev.\
  \textbf{D89} 012004} (2014)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Chatrchyan:2013dma}
CMS collaboration, S.~Chatrchyan {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of a~peaking
  structure in the~$\jpsi\Pphi$~mass spectrum from
  $\decay{\Bu}{\jpsi\Pphi\Kp}$~decays}},
  }{}\href{https://doi.org/10.1016/j.physletb.2014.05.055}{Phys.\ Lett.\
  \textbf{B734} 261--281} (2014)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Chilikin:2013tch}
Belle collaboration, K.~Chilikin {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Experimental constraints on the
  spin and parity of the~\mbox{$\Z\mathrm{(4430)}^+$}}},
  }{}\href{https://doi.org/10.1103/PhysRevD.88.074026}{Phys.\ Rev.\
  \textbf{D88} 074026} (2013)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Belle:2013yex}
Belle collaboration, Z.~Q. Liu {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Study of
  \mbox{$\decay{\epem}{\pip\pim\jpsi}$} and observation of a~charged
  charmoniumlike state at Belle}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.110.252002}{Phys.\ Rev.\ Lett.\
  \textbf{110} 252002} (2013), Erratum
  \href{https://doi.org/10.1103/PhysRevLett.111.019901}{ibid.\   \textbf{111}
  019901} (2013)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Chilikin:2014bkk}
Belle collaboration, K.~Chilikin {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of a~new charged
  charmoniumlike state in \mbox{$\decay{\Bdb}{\jpsi\Km\pip}$}~decays}},
  }{}\href{https://doi.org/10.1103/PhysRevD.90.112009}{Phys.\ Rev.\
  \textbf{D90} 112009} (2014)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2014-014}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of the resonant
  character of the~\mbox{$\PZ(4430)^-$}~state}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.112.222002}{Phys.\ Rev.\ Lett.\
  \textbf{112} 222002} (2014)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2015-029}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of $\jpsi\proton$
  resonances consistent with pentaquark states in
  \mbox{\decay{\Lb}{\jpsi\proton\Km}} decays}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.115.072001}{Phys.\ Rev.\ Lett.\
  \textbf{115} 072001} (2015)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2015-038}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Model-independent confirmation of
  the~\mbox{$\Z(4430)^-$}~state}},
  }{}\href{https://doi.org/10.1103/PhysRevD.92.112009}{Phys.\ Rev.\
  \textbf{D92} 112009} (2015)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2016-018}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of exotic
  $\jpsi\Pphi$~structures from amplitude analysis of
  \mbox{\decay{\Bp}{\jpsi\Pphi\Kp}} decays}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.118.022003}{Phys.\ Rev.\ Lett.\
  \textbf{118} 022003} (2017)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2016-019}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Amplitude analysis of
  \mbox{\decay{\Bp}{\jpsi\Pphi\Kp}} decays}},
  }{}\href{https://doi.org/10.1103/PhysRevD.95.012002}{Phys.\ Rev.\
  \textbf{D95} 012002} (2017)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2018-034}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Evidence for
  a~\mbox{$\Peta_\cquark(1\PS) \pim$}~resonance in
  \mbox{\decay{\Bz}{\Peta_\cquark(1\PS) \Kp\pim}} decays}},
  }{}\href{https://doi.org/10.1140/epjc/s10052-018-6447-z}{Eur.\ Phys.\ J.\
  \textbf{C78} 1019} (2018)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2019-014}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of a~narrow
  pentaquark state, $\PP_\cquark(4312)^+$, and of two-peak structure of
  the~$\PP_\cquark(4450)^+$}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.122.222001}{Phys.\ Rev.\ Lett.\
  \textbf{122} 222001} (2019)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2020-011}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of structure in the
  \jpsi-pair mass spectrum}},
  }{}\href{https://doi.org/10.1016/j.scib.2020.08.032}{Science Bulletin
  \textbf{65} 1983--1993} (2020)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2020-024}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Model\nobreakdash-independent
  study of structure in \mbox{$\decay{\Bp}{\Dp \Dm \Kp}$}~decays}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.125.242001}{Phys.\ Rev.\ Lett.\
  \textbf{125} 242001} (2020)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2020-025}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Amplitude analysis of
  the~\mbox{$\decay{\Bp}{\Dp \Dm \Kp}$}~decay}},
  }{}\href{https://doi.org/10.1103/PhysRevD.102.112003}{Phys.\ Rev.\
  \textbf{D102} 112003} (2020)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2020-035}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Study of \mbox{$\decay{\Bs}{\jpsi
  \pip \pim \Kp \Km}$}~decays}},
  }{}\href{https://doi.org/10.1007/JHEP02(2021)024}{JHEP \textbf{02} 024}
  (2021)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2020-039}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Evidence of a $\jpsi\Lz$
  structure and observation of excited $\Xim$ states in the $\Xibm \rightarrow
  \jpsi \Lz \Km$ decay}},
  }{}\href{https://doi.org/10.1016/j.scib.2021.02.030}{Science Bulletin
  \textbf{66} 1278--1287} (2021)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2020-044}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of new resonances
  decaying into \mbox{$\jpsi\Kp$} and \mbox{$\jpsi\Pphi$}}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.127.082001}{Phys.\ Rev.\ Lett.\
  \textbf{127} 082001} (2021)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Ablikim_2021}
BESIII collaboration, M.~Ablikim {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of
  a~near\nobreakdash-threshold structure in the~\Kp recoil\nobreakdash-mass
  spectra in \mbox{$\decay{\epem}{\Kp\left(\Dsm \Dstarz +
  \D^{*-}_{\squark}\Dz\right) } $} }},
  }{}\href{https://doi.org/10.1103/PhysRevLett.126.102001}{Phys.\ Rev.\ Lett.\
  \textbf{126} 102001} (2021)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2021-018}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Evidence for a~new structure in
  the~$\jpsi\proton$ and $\jpsi\antiproton$~systems
  in~\mbox{$\decay{\Bs}{\jpsi\proton\antiproton}$}~decays}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.128.062001}{Phys.\ Rev.\ Lett.\
  \textbf{128} 062001} (2022)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Brambilla:2019esw}
N.~Brambilla {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{The
  $\PX\PY\PZ$~states: experimental and theoretical status and perspectives}},
  }{}\href{https://doi.org/10.1016/j.physrep.2020.05.001}{Phys.\ Rept.\
  \textbf{873} 1--154} (2020)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{PDG2021}
Particle Data Group, P.~A. Zyla {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{\href{http://pdg.lbl.gov/}{Review
  of particle physics}}}, }{}\href{https://doi.org/10.1093/ptep/ptaa104}{Prog.\
  Theor.\ Exp.\ Phys.\  \textbf{2020} 083C01} (2020), and
  {\href{http://pdglive.lbl.gov/}{2021 update
  {\tt{http:/pdglive.lbl.gov}}}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Oset:2019upy}
E.~Oset {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Tetra and
  pentaquarks from the molecular perspective}},
  }{}\href{https://doi.org/10.1051/epjconf/201919901003}{EPJ Web Conf.\
  \textbf{199} 01003} (2019)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Richard_2016}
J.-M. Richard, \ifthenelse{\boolean{articletitles}}{\emph{Exotic hadrons:
  Review and perspectives},
  }{}\href{https://doi.org/10.1007/s00601-016-1159-0}{Few-Body Systems
  \textbf{57} 1185--1212} (2016)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Guo:2017jvc}
F.-K. Guo {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Hadronic
  molecules}}, }{}\href{https://doi.org/10.1103/RevModPhys.90.015004}{Rev.\
  Mod.\ Phys.\  \textbf{90} 015004} (2018)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{MartinezTorres:2020hus}
A.~Martinez~Torres, K.~P. Khemchandani, L.~Roca, and E.~Oset,
  \ifthenelse{\boolean{articletitles}}{\emph{{Few-body systems consisting of
  mesons}}, }{}\href{https://doi.org/10.1007/s00601-020-01568-y}{Few Body
  Syst.\  \textbf{61} 35} (2020)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Ali:2019roi}
A.~Ali, L.~Maiani, and A.~D. Polosa, {\em {Multiquark Hadrons}},
  \href{https://doi.org/10.1017/9781316761465}{ Cambridge University Press,
  2019}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Ader:1981db}
J.~P. Ader, J.-M. Richard, and P.~Taxil,
  \ifthenelse{\boolean{articletitles}}{\emph{{Do narrow heavy multiquark states
  exist?}}, }{}\href{https://doi.org/10.1103/PhysRevD.25.2370}{Phys.\ Rev.\
  \textbf{D25} 2370--2382} (1982)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Ballot:1983iv}
J.~l. Ballot and J.~M. Richard,
  \ifthenelse{\boolean{articletitles}}{\emph{{Four quark states in additive
  potentials}}, }{}\href{https://doi.org/10.1016/0370-2693(83)90991-7}{Phys.\
  Lett.\  \textbf{B123} 449--451} (1983)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Zouzou:1986qh}
S.~Zouzou, B.~Silvestre-Brac, C.~Gignoux, and J.~M. Richard,
  \ifthenelse{\boolean{articletitles}}{\emph{{Four quark bound states}},
  }{}\href{https://doi.org/10.1007/BF01557611}{Z.\ Phys.\  \textbf{C30}
  457--468} (1986)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Lipkin:1986dw}
H.~J. Lipkin, \ifthenelse{\boolean{articletitles}}{\emph{{A~model-independent
  approach to multiquark bound states}},
  }{}\href{https://doi.org/10.1016/0370-2693(86)90843-9}{Phys.\ Lett.\
  \textbf{B172} 242--247} (1986)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Heller:1986bt}
L.~Heller and J.~A. Tjon, \ifthenelse{\boolean{articletitles}}{\emph{{On
  the~existence of stable dimesons}},
  }{}\href{https://doi.org/10.1103/PhysRevD.35.969}{Phys.\ Rev.\  \textbf{D35}
  969--974} (1987)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Manohar:1992nd}
A.~V. Manohar and M.~B. Wise,
  \ifthenelse{\boolean{articletitles}}{\emph{{Exotic
  $\PQ\PQ\bar{\Pq}\bar{\Pq}$~states in QCD}},
  }{}\href{https://doi.org/10.1016/0550-3213(93)90614-U}{Nucl.\ Phys.\
  \textbf{B399} 17--33} (1993)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2017-018}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of the~doubly charmed
  baryon \Xiccpp}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.119.112001}{Phys.\ Rev.\ Lett.\
  \textbf{119} 112001} (2017)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2018-026}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{First observation of the~doubly
  charmed baryon decay \mbox{\decay{\Xiccpp}{\Xires_c^+\pip}}}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.121.162002}{Phys.\ Rev.\ Lett.\
  \textbf{121} 162002} (2018)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2019-037}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Precision measurement of the
  $\Xiccpp$ mass}}, }{}\href{https://doi.org/10.1007/JHEP02(2020)049}{JHEP
  \textbf{02} 049} (2020)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Karliner:2017qjm}
M.~Karliner and J.~L. Rosner,
  \ifthenelse{\boolean{articletitles}}{\emph{{Discovery of doubly-charmed
  $\Xi_{\cquark\cquark}$ baryon implies a~stable \mbox{$\bquark\bquark
  \uquarkbar \dquarkbar$}~tetraquark}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.119.202001}{Phys.\ Rev.\ Lett.\
  \textbf{119} 202001} (2017)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Carlson:1987hh}
J.~Carlson, L.~Heller, and J.~A. Tjon,
  \ifthenelse{\boolean{articletitles}}{\emph{{Stability of dimesons}},
  }{}\href{https://doi.org/10.1103/PhysRevD.37.744}{Phys.\ Rev.\  \textbf{D37}
  744--753} (1988)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{SilvestreBrac:1993ss}
B.~Silvestre-Brac and C.~Semay,
  \ifthenelse{\boolean{articletitles}}{\emph{{Systematics of \mbox{$L = 0$}
  \mbox{$\quark^2\quarkbar^2$}~systems}},
  }{}\href{https://doi.org/10.1007/BF01565058}{Z.\ Phys.\  \textbf{C57}
  273--282} (1993)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Semay:1994ht}
C.~Semay and B.~Silvestre-Brac,
  \ifthenelse{\boolean{articletitles}}{\emph{{Diquonia and potential models}},
  }{}\href{https://doi.org/10.1007/BF01413104}{Z.\ Phys.\  \textbf{C61}
  271--275} (1994)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Moinester:1995fk}
M.~A. Moinester, \ifthenelse{\boolean{articletitles}}{\emph{{How to search for
  doubly charmed baryons and tetraquarks}},
  }{}\href{https://doi.org/10.1007/s002180050123}{Z.\ Phys.\  \textbf{A355}
  349--362} (1996)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Pepin:1996id}
S.~Pepin, F.~Stancu, M.~Genovese, and J.-M. Richard,
  \ifthenelse{\boolean{articletitles}}{\emph{{Tetraquarks with color blind
  forces in chiral quark models}},
  }{}\href{https://doi.org/10.1016/S0370-2693(96)01597-3}{Phys.\ Lett.\
  \textbf{B393} 119--123} (1997)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{GELMAN2003296}
B.~A. Gelman and S.~Nussinov, \ifthenelse{\boolean{articletitles}}{\emph{{Does
  a~narrow tetraquark $\cquark\cquark\uquarkbar\dquarkbar$~state exist?}},
  }{}\href{https://doi.org/10.1016/S0370-2693(02)03069-1}{Phys.\ Lett.\
  \textbf{B551} 296--304} (2003)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Vijande:2003ki}
J.~Vijande, F.~Fernandez, A.~Valcarce, and B.~Silvestre-Brac,
  \ifthenelse{\boolean{articletitles}}{\emph{{Tetraquarks in a chiral
  constituent quark model}},
  }{}\href{https://doi.org/10.1140/epja/i2003-10128-9}{Eur.\ Phys.\ J.\
  \textbf{A19} 383--389} (2004)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Janc:2004qn}
D.~Janc and M.~Rosina, \ifthenelse{\boolean{articletitles}}{\emph{{The
  $\PT_{\cquark\cquark} = \D\Dstar$ molecular state}},
  }{}\href{https://doi.org/10.1007/s00601-004-0068-9}{Few Body Syst.\
  \textbf{35} 175--196} (2004)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Navarra:2007yw}
F.~S. Navarra, M.~Nielsen, and S.~H. Lee,
  \ifthenelse{\boolean{articletitles}}{\emph{{QCD sum rules study of
  \mbox{$\PQ\PQ-\uquarkbar\dquarkbar$}~mesons}},
  }{}\href{https://doi.org/10.1016/j.physletb.2007.04.010}{Phys.\ Lett.\
  \textbf{B649} 166--172} (2007)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Vijande}
J.~Vijande, E.~Weissman, A.~Valcarce, and N.~Barnea,
  \ifthenelse{\boolean{articletitles}}{\emph{{Are there compact heavy
  four-quark bound states?}},
  }{}\href{https://doi.org/10.1103/PhysRevD.76.094027}{Phys.\ Rev.\
  \textbf{D76} 094027} (2007)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Ebert:2007rn}
D.~Ebert, R.~N. Faustov, V.~O. Galkin, and W.~Lucha,
  \ifthenelse{\boolean{articletitles}}{\emph{{Masses of tetraquarks with two
  heavy quarks in the~relativistic quark model}},
  }{}\href{https://doi.org/10.1103/PhysRevD.76.114015}{Phys.\ Rev.\
  \textbf{D76} 114015} (2007)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Lee:2009rt}
S.~H. Lee and S.~Yasui, \ifthenelse{\boolean{articletitles}}{\emph{{Stable
  multiquark states with heavy quarks in a diquark model}},
  }{}\href{https://doi.org/10.1140/epjc/s10052-009-1140-x}{Eur.\ Phys.\ J.\
  \textbf{C64} 283--295} (2009)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Yang2009}
Y.~Yang, C.~Deng, J.~Ping, and T.~Goldman,
  \ifthenelse{\boolean{articletitles}}{\emph{$\mathrm{S}$-wave
  $\mathrm{QQ}\quarkbar\quarkbar$ state in the~constituent quark model},
  }{}\href{https://doi.org/10.1103/PhysRevD.80.114023}{Phys.\ Rev.\
  \textbf{D80} 114023} (2009)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Li:2012ss}
N.~Li, Z.-F. Sun, X.~Liu, and S.-L. Zhu,
  \ifthenelse{\boolean{articletitles}}{\emph{{Coupled\nobreakdash-channel
  analysis of the~possible \mbox{$\D^{(*)}\D^{(*)}$},
  \mbox{$\Bbar^{(*)}\Bbar^{(*)}$} and \mbox{$\D^{(*)}\Bbar^{(*)}$}~molecular
  states}}, }{}\href{https://doi.org/10.1103/PhysRevD.88.114008}{Phys.\ Rev.\ D
  \textbf{88} 114008} (2013)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Feng:2013kea}
G.-Q. Feng, X.-H. Guo, and B.-S. Zou,
  \ifthenelse{\boolean{articletitles}}{\emph{{$\mathrm{QQ}^{\prime} \uquarkbar
  \dquarkbar$ bound state in the Bethe-Salpeter equation approach}},
  }{}\href{http://arxiv.org/abs/1309.7813}{{\normalfont\ttfamily
  arXiv:1309.7813}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Luo:2017eub}
S.-Q. Luo {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Exotic
  tetraquark states with the $\Pq\Pq\bar{\PQ}\bar{\PQ}$ configuration}},
  }{}\href{https://doi.org/10.1140/epjc/s10052-017-5297-4}{Eur.\ Phys.\ J.\
  \textbf{C77} 709} (2017)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Eichten:2017ffp}
E.~J. Eichten and C.~Quigg,
  \ifthenelse{\boolean{articletitles}}{\emph{{Heavy-quark symmetry implies
  stable heavy tetraquark mesons $\PQ_i\PQ_j \bar \Pq_k \bar \Pq_l$}},
  }{}\href{https://doi.org/10.1103/PhysRevLett.119.202002}{Phys.\ Rev.\ Lett.\
  \textbf{119} 202002} (2017)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Wang:2017uld}
Z.-G. Wang, \ifthenelse{\boolean{articletitles}}{\emph{{Analysis of
  the~axialvector doubly heavy tetraquark states with QCD sum rules}},
  }{}\href{https://doi.org/10.5506/APhysPolB.49.1781}{Acta Phys.\ Polon.\
  \textbf{B49} 1781--1800} (2018)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Park:2018wjk}
W.~Park, S.~Noh, and S.~H. Lee,
  \ifthenelse{\boolean{articletitles}}{\emph{{Masses of the~doubly heavy
  tetraquarks in a~constituent quark model}},
  }{}\href{https://doi.org/10.1016/j.nuclphysa.2018.12.019}{Acta Phys.\ Polon.\
   \textbf{B50} 1151--1157} (2019)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Junnarkar:2018twb}
P.~Junnarkar, N.~Mathur, and M.~Padmanath,
  \ifthenelse{\boolean{articletitles}}{\emph{{Study of doubly heavy tetraquarks
  in Lattice QCD}}, }{}\href{https://doi.org/10.1103/PhysRevD.99.034507}{Phys.\
  Rev.\  \textbf{D99} 034507} (2019)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Deng:2018kly}
C.~Deng, H.~Chen, and J.~Ping,
  \ifthenelse{\boolean{articletitles}}{\emph{{Systematical investigation on the
  stability of doubly heavy tetraquark states}},
  }{}\href{https://doi.org/10.1140/epja/s10050-019-00012-y}{Eur.\ Phys.\ J.\
  \textbf{A56} 9} (2020)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Liu:2019stu}
M.-Z. Liu {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Heavy\nobreakdash-quark spin and
  flavor symmetry partners of the~\mbox{$\PX(3872)$}~revisited: What can we
  learn from the~one boson exchange model?}},
  }{}\href{https://doi.org/10.1103/PhysRevD.99.094018}{Phys.\ Rev.\
  \textbf{D99} 094018} (2019)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Maiani:2019lpu}
L.~Maiani, A.~D. Polosa, and V.~Riquer,
  \ifthenelse{\boolean{articletitles}}{\emph{{Hydrogen bond of QCD in doubly
  heavy baryons and tetraquarks}},
  }{}\href{https://doi.org/10.1103/PhysRevD.100.074002}{Phys.\ Rev.\
  \textbf{D100} 074002} (2019)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Yang:2019itm}
G.~Yang, J.~Ping, and J.~Segovia,
  \ifthenelse{\boolean{articletitles}}{\emph{{Doubly-heavy tetraquarks}},
  }{}\href{https://doi.org/10.1103/PhysRevD.101.014001}{Phys.\ Rev.\
  \textbf{D101} 014001} (2020)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Tan:2020ldi}
Y.~Tan, W.~Lu, and J.~Ping,
  \ifthenelse{\boolean{articletitles}}{\emph{{$\PQ\PQ\bar{\Pq}\bar{\Pq}$ in
  a~chiral constituent quark model}},
  }{}\href{https://doi.org/10.1140/epjp/s13360-020-00741-w}{Eur.\ Phys.\ J.\
  Plus \textbf{135} 716} (2020)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Lu:2020rog}
Q.-F. L\"u, D.-Y. Chen, and Y.-B. Dong,
  \ifthenelse{\boolean{articletitles}}{\emph{{Masses of doubly heavy
  tetraquarks $\PT_{\PQ\PQ^\prime}$ in a relativized quark model}},
  }{}\href{https://doi.org/10.1103/PhysRevD.102.034012}{Phys.\ Rev.\
  \textbf{D102} 034012} (2020)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Braaten:2020nwp}
E.~Braaten, L.-P. He, and A.~Mohapatra,
  \ifthenelse{\boolean{articletitles}}{\emph{{Masses of doubly heavy
  tetraquarks with error bars}},
  }{}\href{https://doi.org/10.1103/PhysRevD.103.016001}{Phys.\ Rev.\
  \textbf{D103} 016001} (2021)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Gao:2020ogo}
D.~Gao {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Masses of
  doubly heavy tetraquark states with isospin = $\frac{1}{2}$ and $1$ and
  spin\nobreakdash-parity~$1^{+\pm}$}},
  }{}\href{http://arxiv.org/abs/2007.15213}{{\normalfont\ttfamily
  arXiv:2007.15213}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Cheng:2020wxa}
J.-B. Cheng {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Double-heavy tetraquark states
  with heavy diquark\nobreakdash-antiquark symmetry}},
  }{}\href{https://doi.org/10.1088/1674-1137/abde2f}{Chin.\ Phys.\ C
  \textbf{45} 043102} (2021)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Noh:2021lqs}
S.~Noh, W.~Park, and S.~H. Lee,
  \ifthenelse{\boolean{articletitles}}{\emph{Doubly heavy tetraquarks,
  ${\Pq}{\Pq}^{\prime}\bar{\PQ}\bar{\PQ}^{\prime}$, in a~nonrelativistic quark
  model with a~complete set of harmonic oscillator bases},
  }{}\href{https://doi.org/10.1103/physrevd.103.114009}{Phys.\ Rev.\
  \textbf{D103} 114009} (2021)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Faustov:2021hjs}
R.~N. Faustov, V.~O. Galkin, and E.~M. Savchenko,
  \ifthenelse{\boolean{articletitles}}{\emph{{Heavy tetraquarks in
  the~relativistic quark model}},
  }{}\href{https://doi.org/10.3390/universe7040094}{Universe \textbf{7} 94}
  (2021)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Ikeda:2013vwa}
Y.~Ikeda {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Charmed
  tetraquarks $\PT_{\cquark\cquark}$ and $\PT_{\cquark\squark}$ from dynamical
  lattice QCD simulations}},
  }{}\href{https://doi.org/10.1016/j.physletb.2014.01.002}{Phys.\ Lett.\
  \textbf{B729} 85--90} (2014)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Cheung:2017tnt}
Hadron Spectrum collaboration, G.~K.~C. Cheung, C.~E. Thomas, J.~J. Dudek, and
  R.~G. Edwards, \ifthenelse{\boolean{articletitles}}{\emph{{Tetraquark
  operators in lattice QCD and exotic flavour states in the charm sector}},
  }{}\href{https://doi.org/10.1007/JHEP11(2017)033}{JHEP \textbf{11} 033}
  (2017)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Francis:2018jyb}
A.~Francis, R.~J. Hudspith, R.~Lewis, and K.~Maltman,
  \ifthenelse{\boolean{articletitles}}{\emph{{Evidence for charm-bottom
  tetraquarks and the mass dependence of heavy-light tetraquark states from
  lattice QCD}}, }{}\href{https://doi.org/10.1103/PhysRevD.99.054505}{Phys.\
  Rev.\  \textbf{D99} 054505} (2019)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-DP-2008-001}
LHCb collaboration, A.~A. Alves~Jr.\ {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{The \lhcb detector at the LHC}},
  }{}\href{https://doi.org/10.1088/1748-0221/3/08/S08005}{JINST \textbf{3}
  S08005} (2008)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-DP-2014-002}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{LHCb detector performance}},
  }{}\href{https://doi.org/10.1142/S0217751X15300227}{Int.\ J.\ Mod.\ Phys.\
  \textbf{A30} 1530022} (2015)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2012-003}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Observation of double charm
  production involving open charm in \proton\proton collisions at
  \mbox{$\sqs=$7\tev}}}, }{}\href{https://doi.org/10.1007/JHEP06(2012)141}{JHEP
  \textbf{06} 141} (2012), Addendum
  \href{https://doi.org/10.1007/JHEP03(2014)108}{ibid.\   \textbf{03} 108}
  (2014)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2021-032}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Study of a~doubly charmed
  tetraquark state}},
  }{}\href{http://arxiv.org/abs/2109.01056}{{\normalfont\ttfamily
  arXiv:2109.01056}}\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2020-008}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Study of the~line shape of
  the~$\chicone(3872)$~state}},
  }{}\href{https://doi.org/10.1103/PhysRevD.102.092005}{Phys.\ Rev.\
  \textbf{D102} 092005} (2020)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2020-009}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Study of the $\psires_2(3823)$
  and $\chicone(3872)$~states in \mbox{$\decay{\Bu}{ \left(
  \jpsi\pip\pim\right)\Kp}$}~decays}},
  }{}\href{https://doi.org/10.1007/JHEP08(2020)123}{JHEP \textbf{08} 123}
  (2020)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PAPER-2013-011}
LHCb collaboration, R.~Aaij {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Precision measurement of \D meson
  mass differences}}, }{}\href{https://doi.org/10.1007/JHEP06(2013)065}{JHEP
  \textbf{06} 065} (2013)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\end{mcitethebibliography}


==> refs_methods.tex <==
\ifx\mcitethebibliography\mciteundefinedmacro
\PackageError{LHCb.bst}{mciteplus.sty has not been loaded}
{This bibstyle requires the use of the mciteplus package.}\fi
\providecommand{\href}[2]{#2}
\begin{mcitethebibliography}{100}
\mciteSetBstSublistMode{n}
\mciteSetBstMaxWidthForm{subitem}{\alph{mcitesubitemcount})}
\mciteSetBstSublistLabelBeginEnd{\mcitemaxwidthsubitemform\space}
{\relax}{\relax}

\bibitem{LHCb-DP-2012-003}
M.~Adinolfi {\em et~al.},
  \ifthenelse{\boolean{articletitles}}{\emph{{Performance of the \lhcb RICH
  detector at the LHC}},
  }{}\href{https://doi.org/10.1140/epjc/s10052-013-2431-9}{Eur.\ Phys.\ J.\
  \textbf{C73} 2431} (2013)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PROC-2010-056}
I.~Belyaev {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{Handling
  of the generation of primary events in {\sc{Gauss}}, the LHCb simulation
  framework}}, }{}\href{https://doi.org/10.1088/1742-6596/331/3/032047}{J.\
  Phys.\ Conf.\ Ser.\  \textbf{331} 032047} (2011)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Lange:2001uf}
D.~J. Lange, \ifthenelse{\boolean{articletitles}}{\emph{{The~{\sc{EvtGen}}
  particle decay simulation package}},
  }{}\href{https://doi.org/10.1016/S0168-9002(01)00089-4}{Nucl.\ Instrum.\
  Meth.\  \textbf{A462} 152--155} (2001)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{LHCb-PROC-2011-006}
M.~Clemencic {\em et~al.}, \ifthenelse{\boolean{articletitles}}{\emph{{The
  \lhcb simulation application, {\sc{Gauss}}: Design, evolution and
  experience}}, }{}\href{https://doi.org/10.1088/1742-6596/331/3/032023}{J.\
  Phys.\ Conf.\ Ser.\  \textbf{331} 032023} (2011)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Hulsbergen:2005pu}
W.~D. Hulsbergen, \ifthenelse{\boolean{articletitles}}{\emph{{Decay chain
  fitting with a Kalman filter}},
  }{}\href{https://doi.org/10.1016/j.nima.2005.06.078}{Nucl.\ Instrum.\ Meth.\
  \textbf{A552} 566--575} (2005)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\bibitem{Pivk:2004ty}
M.~Pivk and F.~R. Le~Diberder,
  \ifthenelse{\boolean{articletitles}}{\emph{{sPlot: A statistical tool to
  unfold data distributions}},
  }{}\href{https://doi.org/10.1016/j.nima.2005.08.106}{Nucl.\ Instrum.\ Meth.\
  \textbf{A555} 356--369} (2005)\relax
\mciteBstWouldAddEndPuncttrue
\mciteSetBstMidEndSepPunct{\mcitedefaultmidpunct}
{\mcitedefaultendpunct}{\mcitedefaultseppunct}\relax
\EndOfBibitem
\end{mcitethebibliography}

